KF-CS: Compressive Sensing on Kalman Filtered Residual

We consider the problem of recursively reconstructing time sequences of sparse signals (with unknown and time-varying sparsity patterns) from a limited number of linear incoherent measurements with additive noise. The idea of our proposed solution, KF CS-residual (KF-CS) is to replace compressed sensing (CS) on the observation by CS on the Kalman filtered (KF) observation residual computed using the previous estimate of the support. KF-CS error stability over time is studied. Simulation comparisons with CS and LS-CS are shown.

==> figs8.tex <==
\begin{figure*}[t!]
\centerline{
\subfigure[comparison with simple CS]{
\label{CScompare}
%\begin{tabular}{c}
\epsfig{file = C:/Code/KFCS/mse_normalized_without_del_CS_2newadds_2.eps, height = 3cm,width=5cm}
%\end{tabular}
}
\subfigure[LS/KF CS-res LS/KF]{
\label{algos_compare}
%\begin{tabular}{c}
\epsfig{file = C:/Code/KFCS/mse_normalized_without_del_2newadds_genie.eps, height =3cm,width=5cm}
}
\subfigure[KF-CS-res-LS with/without deletion]{
\label{deletion_compare}
\epsfig{file = C:/Code/KFCS/mse_normalized_with_without_del_2newadds_kfcsls.eps, height = 3cm,width=5cm}
%\end{tabular}
}
}
\centerline{
\subfigure[mean no. false additions, $\Nhat_{t-1} \setminus N_t$]{
\label{mean_fa}
%\begin{tabular}{c}
\epsfig{file = C:/Code/KFCS/num_false_adds_2newadds.eps , height = 3cm,width=5cm}
}
\subfigure[mean no. of misses, $N_t \setminus \Nhat_{t}$]{
\label{mean_misses}
\epsfig{file = C:/Code/KFCS/num_misses_2newadds.eps, height = 3cm,width=5cm}
%\end{tabular}
}
\subfigure[model 2: comparison with simple CS]{\label{model2}
\epsfig{file = C:/Code/KFCS/mse_normalized_with_del_CS_4newadds.eps, height = 3cm,width=5cm}
%\end{tabular}
}
}
\caption{\small{Comparing CS and different versions of CS-residual.
All plots except Fig. \ref{model2} are for the first model ($S_1=8$, 2 new additions every 5 time units from $t=10$ to $50$). Fig. \ref{model2} is for the second model ($S_1=8$, 4 new additions every 10 time units from $t=10$ to $30$).%
}}
\label{fig}
\end{figure*}



==> figures_2.tex <==

%\begin{tabular}{|c|c|c|c|c|}
%\hline
% & $\sigma$ = 0.04 &  $\sigma$ = 0.09 &  $\sigma$ = 0.18 & $\sigma$=0.44 \\
% \hline
%Dantzig, $\lambda=4\sigma$ &&&& \\
%\hline
%Dantzig, $\lambda=0.4\sigma$ &&&& \\
%\hline
%Gauss-Dantzig &&&& \\
%\hline
%CS-residual, $\lambda=4\sigma$ &&&& \\
%\hline
%LS-CS &&&& \\
%\hline
%\end{tabular}



\begin{figure}[b!]
\vspace{-0.2in}
\centerline{
\epsfig{file = ../figs/stability_n_59_final_CS_subplot2.eps, width=8cm}
}
\vspace{-0.2in}
\caption{\small{{\em Verifying the Stability Result} for Signal Model \ref{sigmod1} with $d=8$, $r=2$, $M=3$, and with $a_i$ either 0.5 or 0.25. Notice that LS-CS stabilizes to the genie-LS within 4 time units. Also notice that the LS-CS error is less than 0.4\% at all times while CS error is 30-40\%.%. We simulated a signal sequence according to Signal Model \ref{sigmod2} with $d=8$, $r=2$, $M=3$, and with half of all the $a_i$'s being 0.5 and the other half being 0.25. Also, $m=200$, $S_0=20$, $S_a=2$. We used  $n=59$ and noise was $unif(-c,c)$ with $c= 0.0528$. LS-CS was run with $\alpha=c$, $\alpha_{del}=2.28c$ and $\lambda = c \|A\|_1$. We averaged over 100 simulations. In our simulations, $d_0$ was at most 3, i.e. within at most $d_0+S_a-1=4$ time units after a new addition, $\Nhat_t=N_t$, i.e. LS-CS=genie-LS. CS-residual: $\lambda=0.176$, Dantzig: $\lambda=0.0176$.
}}
\label{stability_fig}
\end{figure}



\begin{figure*}[t!]
\centerline{
\subfigure[Low SNR, Slow adds, $n$=59]{% Slow adds/dels,
\label{kfcs_better_59}
%\begin{tabular}{c}
%\epsfig{file = ../figs/kfcs_better_n_59_sigmodel2_error.eps, height = 3cm,width=4cm}
\epsfig{file = ../figs/kfcs_better_sigmodel2_run_init_cs_n_59_error.eps, height = 3cm,width=4cm}
%\end{tabular}
}
\subfigure[Low SNR, Slow adds, $n$=40]{
\label{kfcs_better_40}
%\begin{tabular}{c}
\epsfig{file = ../figs/kfcs_better_sigmodel2_run_init_cs_n_40_error.eps, height = 3cm,width=4cm}
%\end{tabular}
}
\subfigure[Low SNR, Fast adds, $n$=59]{
\label{fast_adds_dels}
%\begin{tabular}{c}
\epsfig{file = ../figs/fast_adds_dels_error.eps, height = 3cm,width=4cm}
%\end{tabular}
}
\subfigure[CS plots corresp. to Fig.\ref{kfcs_better_59}]{
\label{CS_kfcs_better_59}
%\begin{tabular}{c}
\epsfig{file=../figs/kfcs_better_n_59_sigmodel2_run_init_cs_error_CS.eps, height = 3cm,width=4cm}
%\epsfig{file = C:/Code/KFCS/mse_normalized_without_del_CS_2newadds_final.eps, height = 3cm,width=4cm}
%\end{tabular}
}
}
\centerline{
\subfigure[Low SNR, Slow adds, $n$=59]{% Slow adds/dels,
\label{kfcs_better_59_support}
%\begin{tabular}{c}
%\epsfig{file = ../figs/kfcs_better_n_59_sigmodel2_error.eps, height = 3cm,width=4cm}
\epsfig{file = ../figs/kfcs_better_sigmodel2_run_init_cs_n_59_misses_extras.eps, height = 3cm,width=4cm}
%\end{tabular}
}
\subfigure[Low SNR, Slow adds, $n$=40]{
\label{kfcs_better_40_support}
%\begin{tabular}{c}
\epsfig{file = ../figs/kfcs_better_sigmodel2_run_init_cs_n_40_misses_extras.eps, height = 3cm,width=4cm}
%\end{tabular}
}
\subfigure[Low SNR, Fast adds, $n$=59]{
\label{fast_adds_dels_support}
%\begin{tabular}{c}
\epsfig{file = ../figs/fast_adds_dels_misses_extras.eps, height = 3cm,width=4cm}
%\end{tabular}
}
\subfigure{%[Signal Model \ref{randomwalk}]{
\label{oldsim}
\epsfig{file=../figs/kfcs_better_n_59_sigmodel2_run_init_cs_error_CS.eps, height = 3cm,width=4cm}
%%\begin{tabular}{c}
%%\epsfig{file = C:/Code/KFCS/mse_normalized_without_del_CS_2newadds_final.eps, height = 3cm,width=4cm}
%\epsfig{file = ../figs/mse_normalized_without_del_2newadds_genie_final.eps, height = 3cm,width=4cm}
%%\end{tabular}
}
}
\caption{\small{Lower SNR simulations. Comparing LS-CS and KF-CS. CS-residual used $\lambda=0.17$ for LS-CS and KF-CS.
Fig. \ref{CS_kfcs_better_59} gives the CS plot corresponding to Fig.\ref{kfcs_better_59} for two choices of $\lambda$.%0.1757
%Fig. \ref{oldsim} simulates the random walk model with increase support size (Signal Model \ref{randomwalk}).% This used $n=72$, $m=256$, $S_0=8$.
%In \ref{fast_adds_dels}, additions/deletions occur every $d=3$ time units. KF-CS does not get a chance to stabilize. Because it retains memory of past estimates, its errors are larger at new addition times. In \ref{kfcs_better_59}, additions/deletions occur every $d=8$ time units. Once all get detected, KF-CS is able to stabilize to a value smaller than LS-CS and the genie-LS. In \ref{kfcs_better_40}, everything is same as above, but we use $n=40$. This is too small and $A_T'A_T$ often becomes badly conditioned, causing LS-CS error to increase over time. KF-CS remains stable because of it uses past information. We also run the initial CS step in the last three figures.
}}
\vspace{-0.2in}
\label{lscs_kfcs}
\end{figure*}




==> introduction_revise.tex <==
%For a single spatial signal, the solution is provided by Compressed Sensing (CS). The question that we ask is: for a time sequence of sparse signals, how can we improve the accuracy of simple CS (CS at each time separately) by using past observations and how can we do it recursively, i.e. by only using the previous signal estimate and the current observation.
\begin{abstract}%, {\em in real-time}
We consider the problem of recursively reconstructing time sequences of sparse signals (with unknown and time-varying sparsity patterns) from a limited number of linear incoherent measurements with additive noise. The signals are sparse in some transform domain referred to as the sparsity basis and the sparsity pattern is assumed to change slowly with time. The idea of our proposed solution, LS-CS-residual (LS-CS), is to replace compressed sensing (CS) on the observation by CS on the least squares (LS) observation residual computed using the previous estimate of the support. We bound the CS-residual error and show that when the number of available measurements is small, the bound is much smaller than that on CS error if the sparsity pattern changes slowly enough. We also obtain conditions for ``stability" of LS-CS over time for a simple deterministic signal model of coefficient addition/removal and coefficient magnitude increase/decrease which has bounded signal power. By ``stability", we mean that the number of misses and extras in the support estimate is bounded by a small value compared to the support size,  at all times. Extensive simulation results backing our claims are shown.%
%Kalman filtered CS-residual (KF-CS), which replaces the LS residual by a Kalman filtered (Bayesian LS) residual, is also proposed.% and briefly studied.%We also obtain the conditions under which the KF CS-residual estimate eventually converges to that of the genie-aided KF (the KF that knows the support at each time). A useful corollary is that if the sparsity pattern changes slowly enough, the KF CS-residual estimate stabilizes to within a small error of the genie-aided KF estimate.%, in probability  (CS-residual)  (and thus bounded SNR).
\end{abstract}
%\vspace{-0.1in}


%{\bf Keywords:} compressed sensing, kalman filter, least squares% estimation% sparse signal sequence estimation,
%imaging of brain neural activation patterns in response to varying stimuli. This capability is critical to making MR image guided surgery or other interventional MRI applications practical \cite{interventionalMR}.

\Section{Introduction} % of recursive sparse reconstruction problems  or pressure of the beating heart or
\label{intro}

Consider the problem of recursively and causally reconstructing time sequences of spatially  sparse signals (with unknown and time-varying sparsity patterns) from a limited number of linear incoherent measurements with additive noise. The signals are sparse in some transform domain referred to as the ``sparsity basis" \cite{decodinglp}. An important example of such a problem is dynamic magnetic resonance (MR) image reconstruction of deforming brain shapes in real-time applications such as MR image guided surgery or functional MRI \cite{interventionalMR}. %; or real-time functional MRI applications. %of neuronal activation patterns.
 Human organ images are piecewise smooth and so the wavelet transform is a valid sparsity basis \cite{sparseMRI}. MRI captures a limited number of Fourier coefficients of the image, which are incoherent with respect to the wavelet transform \cite{dantzig,sparseMRI}. Other examples include real-time estimation of time-varying spatial fields using sensor networks \cite{nowaknoise} or real-time single-pixel video imaging \cite{singlepixel}, or video compression.
%of time varying spatial fields using a network of sensors that transmit using the random projection protocol of \cite{nowaknoise}; real-time video reconstruction/display using single-pixel camera \cite{singlepixel}, or video compression. %, such as temperature change in a large area,  energy-efficient random projection sensing  usually
%Due to strong temporal dependencies, the sparsity pattern usually changes {\em slowly} over time. that are usually at least second order Markovian,
Due to strong temporal dependency in the signal sequence, it is usually valid to assume that its {\em sparsity pattern (support of the sparsity transform vector) changes slowly over time}, except in case of sudden scene change. This was empirically verified in \cite{kfcsmri}. %for dynamic MRI.%This was observed by us in \cite{icipmodcs}.%
%This was empirically observed in our medical image sequence experiments in \cite{icipmodcs}.% Both are sparse in the wavelet domain and the maximum size of the change in sparsity pattern is less than 3\% of the minimum support size at any time.% [see Fig. \ref{MRIplots}].with cardiac and brain image sequences  empirically

%CS for noise-free observations \cite{candes,decodinglp} is exact with high probability (w.h.p.), while
The solution to the static version of the above problem is provided by compressed sensing (CS) \cite{candes,donoho}. CS for noisy observations, e.g. Dantzig selector  \cite{dantzig} or Basis Pursuit Denoising (BPDN) \cite{bpdn,tropp}, have been shown to have small error as long as incoherence assumptions hold.  Most existing solutions for the dynamic problem, e.g. \cite{singlepixel,sparsedynamicMRI}, are non-causal and batch solutions. Batch solutions process the entire time sequence in one go and thus have much higher reconstruction complexity. An alternative would be to apply CS at each time separately (simple CS), which is online and low-complexity, but since it does not use past observations, its reconstruction error is much larger when the number of available observations is small.
 %
%With the exception of \cite{rozell,jung_etal}, most existing solutions for the dynamic problem, e.g. \cite{singlepixel,sparsedynamicMRI}, jointly reconstruct the entire sequence of signals in one go. This is a non-causal or batch solution with very high reconstruction complexity. An alternative would be to apply CS at each time separately, which is online and low-complexity, but since it does not use past observations, its reconstruction error is much larger, particularly when the number of available measurements is small. We refer to this approach as {\em simple CS}.% in this paper.% (assume Fourier sparsity along the time axis and wavelet sparsity of the spatial signal/image)  at a given time (e.g. Dantzig selector)
%
 %(or equivalently, it will require many more measurements to achieve low error).
%The question that we address is:  {\em can we do better than performing CS at each time separately, if (a) the sparsity pattern (support set) of the transform coefficients' vector changes slowly, i.e. every time, none or only a few elements of the support change, and (b) a prior model on the temporal dynamics of its current non-zero elements is available}.% (but do not know  (need to wait to get the entire observation sequence) and has
%
% %If the previous support estimate is accurate and if the sparsity pattern changes slowly enough, the residual measures a signal whose approximate sparsity size is much smaller than that of the original signal. As a result, the reconstruction error using CS-residual is much smaller than that of simple CS, particularly when the number of observations is small.  use this idea to
%
The question is: for a time sequence of sparse signals, how can we obtain a recursive solution that improves the accuracy of simple CS by using past observations? By {\em ``recursive", we mean a solution that uses only the previous signal estimate and the current observation vector at the current time.} %, when the number of available observations at a given time is small, and how can we do it {\em recursively, i.e. by only using the previous signal estimate and the current observation}.
The key idea of our solution is to replace CS on the observation by CS on the least squares (LS) residual computed using the previous support estimate. Its complexity is equal to that of simple CS which is $O(Nm^3)$ where $m$ is the signal length and $N$ is the time duration \cite[Table 1]{ldpc_cs}. Compare this to $O(N^3m^3)$ for a batch solution.%
%%Our conference papers \cite{kfcsicip,kfcspap} were the first to provide a recursive CS solution.
%We bound CS-residual error and compare it to that of simple CS error. We also obtain conditions for stability of the complete LS CS-residual (LS-CS) algorithm  over time for simple deterministic model of coefficient increase/decrease. Kalman filtered CS-residual (KF-CS), which replaces the initial LS estimate by a Bayesian LS (Kalman filtered) estimate, is proposed and briefly studied.
% (simple CS)
%Note that LS CS-residual is also applicable to a static CS problem when part of the support is known from some ``prior knowledge".%, e.g. if an image contains no black background, the indices of the lowest frequency subband of wavelet coefficients will be contained in the support. This could serve as the ``known" part of the support.% and its bounds are
 %,model-CS,TOMP_do}.  and model-based %work in literature that also uses statistical models , or Bayesian LS (Kalman filtered),

%they do not use it to reduce the number of measurements required for the current reconstruction and homotopy methods } and the very recent work of \cite{  ,priorCS  \cite{imagereconcs} (uses a recursive algorithm)
Other related work includes \cite{rozell,romberg}, which use the previous estimate and/or homotopy to speed up the current optimization, but not to improve reconstruction error, and \cite{giannakis} which also addresses recursive sparse estimation but with time-invariant support. Both \cite{romberg}, \cite{giannakis} appeared after \cite{kfcsicip}. The work of \cite{jung_etal} (k-t-focuss) gives a faster but approximate batch solution for dynamic MRI. Some other related work, but all for reconstructing a single sparse signal, includes \cite{bayesianCS,schniter,ldpc_cs} (Bayesian approaches), \cite{imagereconcs} (uses a recursive algorithm) and \cite{distCS} (related model, but offline algorithm).

%if the different sources in distributed CS are replaced by different time instants, this provides another offline solution to our problem)
%exploits spatial correlation between temporal signals from various sources).%,distCS}. The model used by \cite{schniter} is discussed further in Sec. \ref{conclusions}.%Bayesian approaches for sp to for a single signal are proposed in \cite{bayesianCS,priorCS,schniter,ldpc_cs}, while
%Bayesian approaches to sparse reconstruction of a single signal include \cite{bayesianCS,priorCS,schniter,ldpc_cs,imagereconcs}. The model used by \cite{schniter} is discussed further in Sec. \ref{conclusions}.%,distCS

\Subsection{Paper Organization and Important Sections}
We give the notation and problem definition in the next two subsections. The CS-residual idea and the complete LS-CS algorithm are developed in Sec. \ref{lscs}. We bound its error at a given time instant and compare it with CS in Sec. \ref{csresbound}. Conditions for stability of LS-CS, under a deterministic model of coefficient increase/decrease, are obtained in Sec. \ref{stability}. %KF-CS is developed Sec. \ref{kfcs}.
Simulation results are given in Sec. \ref{sims} and conclusions in Sec. \ref{conclusions}. %The {\em main ideas of this work} are given in Sections \ref{lscs}, \ref{csresbound1}, \ref{comparecs}, \ref{stability} and \ref{sims}.
Sections/subsections marked with ** can be skipped on a quick reading.

 In this work, we do ``CS", whether in simple CS or in CS-residual, using the Dantzig selector \cite{dantzig}. This choice was initially motivated by the fact that its guarantees are stronger (depend only on signal support size, not support elements) than those for BPDN \cite{tropp} and its results are simpler to apply and modify. In later work \cite{kfcsmri}, we have also used BPDN.%basis pursuit denoising (BPDN)


%The main ideas of this work are given in Section \ref{lscs} (algorithm), Sections \ref{csresbound1}, \ref{comparecs} (CS-residual error bound and comparison with CS), Section \ref{stability} (LS-CS stability) and Section \ref{sims} (simulations). Sections marked with ** can be skipped on a quick reading.%

%The key idea of our approach is given in Sections \ref{intro}, \ref{lscs}. Sections \ref{csresbound1}, \ref{comparecs} (CS-residual error bound),  Section \ref{stabres1} (basic LS-CS stability result)  and Section \ref{sims} (simulations) give the most important theoretical and numerical evidence of why our approach works.

% since it runs faster.% (unconstrained optimization).

%\Subsection{Related Work}


%dominant basis  We refer to this solution as genie-aided KF.
%Kalman filtered CS-residual may also be understood as an approximate solution to the problem of causal minimum mean squared error (MMSE) estimation with a slow time-varying set of directions of variability in the transform domain (or equivalently the support set of the transform vector). If the support is known at each time, the MMSE solution is given by a reduced-order Kalman filter (KF) \cite{ekf} implemented for the current set of nonzero coefficients. If the support set is unknown and time-varying, we can do the following. We use CS to estimate the initial signal and its support. At future times we run KF on the current support estimate. We use CS on the KF residual to find new additions, if any, to the support at each time. In this work, we show that the KF CS-residual estimate eventually converges to that of the genie-aided KF. A useful corollary is that if the sparsity pattern changes slowly enough, KF CS-residual stabilizes to within a small error of the genie-aided KF. An analogous result holds for LS CS-residual. % (the KF that knows the support at each time) under certain assumptions  estimate
%changes slowly with time and  if all additions to the support occur before a certain finite time,

%We give the problem definition in Sec. \ref{problem}. LS and KF CS-residual are described in Sec. \ref{algos}. We bound LS CS-residual error in Sec. \ref{cslseanal}. Convergence to genie-aided KF (or LS), and the corresponding corollaries are derived in Sec. \ref{converge}. Simulation comparisons are given in Sec. \ref{sims} and discussion in Sec. \ref{discuss}.%
%. The limitations of our results are discussed in Sec. \ref{discuss}.%implications and  of KF-CS-residual (resp. LS-CS-residual)  implications




%Let $T$ denote the previous estimate of the support and let $\Delta$ be the unknown part of the current support, i.e. the current support is $T \cup \Delta$. The reason CS-residual outperforms
%Our preliminary analysis and simulations indicate that it has significantly smaller reconstruction error than simple CS, particularly when number of available measurements is small. %The reason is that it tries to reconstruct a ``signal" that is only $|\Delta|$-approximately sparse (where $\Delta$ is the current support minus its estimate from the previous time). %When measurements are noisy, our preliminary analysis and simulations indicate that the {\em bounds on CS-residual error are much smaller than those on simple CS error}.



==> problem_formulation.tex <==

%\section{Notation and Problem Definition} \label{problem}

\Subsection{Notation}
\label{notation}
%$m$ denotes the signal length while $n$ denotes the number of measurements used at $t>0$.

The set operations $\cup$, $\cap$, and $\setminus$ have the usual meanings. $T^c$ denotes the complement of $T$ w.r.t. $[1,m]:=[1,2,\dots m]$, i.e. $T^c := [1,m] \setminus T$. $|T|$ denotes the size (cardinality) of $T$.%$\phi$ refers to the empty set.

For a vector, $v$, and a set, $T$, $v_T$ denotes the $|T|$ length sub-vector containing the elements of $v$ corresponding to the indices in the set $T$. $\|v\|_k$ denotes the $\ell_k$ norm of a vector $v$. If just $\|v\|$ is used, it refers to $\|v\|_2$. Also, $v_{(i)}$ refers to the $i^{th}$ largest {\em magnitude} element of $v$ (notation taken from \cite{decodinglp}). Thus, for an $m$ length vector, $|v_{(1)}| \ge |v_{(2)}| \dots \ge |v_{(m)}|$.%

We use the notation $v(S)$ to denote the sub-vector of $v$ containing the $S$ smallest magnitude elements of $v$.

For a matrix $M$, $\|M\|_k$ denotes its induced $k$-norm, while just $\|M\|$ refers to $\|M\|_2$. $M'$ denotes the transpose of $M$. For a tall matrix, $M$, $M^\dag : = (M'M)^{-1}M'$.

For a fat matrix $A$, $A_T$ denotes the sub-matrix obtained by extracting the columns of $A$ corresponding to the indices in $T$.
The $S$-restricted isometry constant \cite{decodinglp}, $\delta_S$, for an $n \times m$ matrix (with $n<m$), $A$, is the smallest real number satisfying
\bea
(1- \delta_S) \|c\|^2 \le \|A_T c\|^2 \le (1 + \delta_S) \|c\|^2
\label{def_delta}
\eea
for all subsets $T \subset [1,m]$ of cardinality $|T| \le S$ and all real vectors $c$ of length $|T|$. %It is easy to see that $\|A_T'A_T\| \le (1 + \delta_S)$ and $\|(A_T'A_T)^{-1}\| \le 1/(1- \delta_S)$.
The restricted orthogonality constant \cite{decodinglp}, $\theta_{S,S'}$, is the smallest real number satisfying
\bea
| {c_1}'{A_{T_1}}'A_{T_2} c_2 | \le \theta_{S,S'} \|c_1\| \|c_2\| %\ \text{whenever} \ \|v_1\|_0 \le S  \ \text{and}   \ \|v_2\|_0 \le S'
\label{def_theta}
\eea
for all disjoint sets $T_1, T_2 \subset [1,m]$ with $|T_1| \le S$, $|T_2| \le S'$, $S+S' \le m$, and for all vectors $c_1$, $c_2$ of length $|T_1|$, $|T_2|$.% respectively %By setting $c_1 = {A_{T_1}}'A_{T_2} c_2$ in (\ref{def_theta}), it is easy to see that  $\|{A_{T_1}}'A_{T_2}\| \le \theta_{S,S'}$.

For a square matrix, $Q$, we use $(Q)_{T_1,T_2}$ to denote the sub-matrix of $Q$ containing rows and columns corresponding to the entries in $T_1$ and $T_2$ respectively. $I$ denotes an appropriate sized identity matrix.
{\em The $m \times m$ matrix $I_T$ is defined as}
\bea
(I_T)_{T,T} = I, \ (I_T)_{T^c,[1,m]} = 0, \ (I_T)_{[1,m], T^c} = 0
\label{defI}
\eea
%where $I$ is a $|T|$-identity matrix.
% while  $(I_T)_{T^c,[1,m]} = \mathbf{0}$,  $(I_T)_{[1,m], T^c} = \mathbf{0}$.}




%Let $N_t$ denote the support set of $x_t$, i.e. the set of its non-zero coordinates and let $S_t : = |N_t|$. Let $\hat{N}_t$ denote the estimate of $N_t$. Also, let $\Delta_t$ denote the undetected part of the support at $t$, i.e.  $\Delta_t \defn N_t \setminus \Nhat_{t-1}$ and let $\hat{\Delta}_t$ denote its estimate.% Thus $\Nhat_t = \Nhat_{t-1} \cup \hat{\Delta}_t$.
%$T_t = T_{t-1} \cup \hat{\Delta}_t$.


\Subsection{Problem Definition and Some More Notation}
\label{probdef}
Let $(z_t)_{m \times 1}$ denote the spatial signal at time $t$ and $(y_t)_{n \times 1}$, with $n<m$, denote its noise-corrupted observation vector at $t$, i.e. $y_t = H z_t + w_t$. The signal, $z_t$, is sparse in a given sparsity basis (e.g. wavelet) with orthonormal basis matrix, $\Phi_{m \times m}$, i.e. $x_t \defn \Phi' z_t$ is a sparse vector. We denote its support by $N_t$ and we use $S_t:= |N_t|$ to denote its size. Sparse means that $S_t  \ll  m$. %Here, $H$ is the measurement matrix. %, e.g. a (random $\pm 1$ matrix) i %(e.g. randomly selected rows of a discrete Fourier transform (DFT) matrix in case of MR imaging).  Here $'$ denotes transpose.
Thus the observation model is
\bea
y_t = A x_t + w_t, \ A \defn H \Phi, \ \  \E[w_t]=0, \  \E[w_t w_t']= \sigma^2 I \ \ \ \
 %w_t \sim \n(0,\sigma_{obs}^2 I) %\underbrace{H \Phi}_
\label{obsmod}
\eea
%$H$ is s.t.  (or less) and all $S_t$ column sub-matrices of $A \defn H \Phi$ are ``approximately orthonormal" \cite{dantzig}.  $H$ is the measurement matrix (e.g. randomly selected rows of a Fourier matrix in case of MR imaging).
We assume that $A$ has unit norm columns. The observation noise, $w_t$, is independent identically distributed (i.i.d.) over $t$ and is independent of $x_t$. Our goal is to recursively obtain the best estimates of $x_t$ (or equivalently of the signal, $z_t = \Phi x_t$) using $y_1, \dots y_t$. By {\em recursively}, we mean, use only $y_t$ and the estimate from $t-1$, $\xhat_{t-1}$, to compute the estimate at $t$.

We assume that the sparsity pattern (support) of $x_t$ changes ``slowly" over time. Also the observations are assumed to be incoherent w.r.t. the sparsity basis of the signal, i.e. all $S$-column sub-matrices of $A \defn H \Phi$ are ``approximately orthonormal" (have all nonzero singular values close to 1) \cite{dantzig}, for $S$ a little more than $S_t$. We quantify both the above assumptions after giving the following definition.
%, i.e. $\delta_S = \delta_S(A) < 1$

\bd[Define $\sone$, $\sinf$]
For $A:=H \Phi$, %define the following two quantities:
\ben
\label{deltas}
\item let $\sone$ denote the largest $S$ for which $\delta_S < 1/2$,
\label{delta3s}
\item let $\sinf$ denote the largest $S$ for which $\delta_{2S}+ \theta_{S,2S} < 1$.%\gamma \le
\een
%(the choice 1/2 in \ref{deltas}) is arbitrary, we can use any $b<1$)
\label{delta_bnd}
\ed
\begin{ass}
Assume that
%The following assumptions are used in the entire paper.
%Our algorithm relies on the following.
%In the entire paper, we assume the following. %about $A$ and about sparsity
\ben
\item The additions at any time, $|N_t \setminus N_{t-1}| \le S_a  \ll  S_t$ and the removals, $|N_{t-1} \setminus N_t| \le S_r  \ll  S_t$.% Typically $S_a  \approx S_a$. %Knowledge of $S_a$ or $S_r$ is not needed by the algorithm.%
\item $A$ satisfies $S_t + S_r < \sone$ and $S_a < \sinf$.
\een
\label{initass}
\end{ass}
The slow support change assumption was empirically verified in our recent work \cite{kfcsmri}. We observed that typically $S_a \approx S_r \le S_t/10$, and $S_t$ stays roughly constant. Approximate orthonormality is known to hold with high probability (w.h.p.) when $A$ is a random Gaussian, Rademacher or partial Fourier matrix and $n$ is large enough \cite{decodinglp,dantzig}.
%is approximately orthonormal, i.e.

\subsubsection{More Notation}% (we explain how this is computed later)
We use $\xhat_t$ to denote the estimate of $x_t$ given by our algorithm at time $t$ and $\Nhat_t$ to denote its support estimate. To keep notation simple, we avoid using the subscript $t$ wherever possible. We will use the following sets often.%
\bd[Define $T$, $\Delta$, $\Delta_e$]
We use $T  : = \Nhat_{t-1}$ to denote the support estimate from the previous time. This serves as an initial estimate of the current support.% =T(t)
We use $\Delta := N_t \setminus T$ to denote the unknown part of the support at the current time. % =\Delta(t)
We use $\Delta_e := T \setminus N_t$ to denote the ``erroneous" part of $T$.
\ed
\bd[Define $\tT$, $\tDelta$, $\tDelta_e$]
We use $\tT := \Nhat_t$ to denote the final estimate of the current support.
We use $\tDelta : = N_t \setminus \tT$ to denote the ``misses" in the final estimate and $\tDelta_e := \tT \setminus N_t$ to denote the ``extras". %(extra elements that wrongly got added). (elements of the current support which did not get detected by the algorithm)
\ed

Some more notation - $\xhat_{\CSres}$, $\tDelta_{\dett}$, $\tT_{\dett}$, $\alpha$, $\alpha_{del}$, -  is defined when we give our algorithm in Sec. \ref{lscs}. %(again all of these should have the subscript $t$) $\xhat_{\dett}$, $\Nhat_{\dett}$,



%Assume that the measurement matrix $A:=H \Phi$ satisfies
%\ben
%%\item $\delta_S < \defb < 1$ for all $1 \le S \le \sone$ (e.g. $b=1/2$)
%\label{deltas}
%\item $\delta_S < \defb$ for all $1 \le S \le \sone$,%
%\label{delta3s}
%\item $\delta_{2S}+ \theta_{S,2S} < 1$ for all $1 \le S \le \sinf$ (clearly $\sinf \le \sone$),%
%%\item  $\smax < \sone$ and $\samax < \sinf$.
%\een
%%$\theta_{S,S'}$ is defined in \cite[eq. (1.5)]{dantzig}.
%%$\delta_{\smax + S_{fa}}< 1$. $\delta_S = \delta_S(A)$ is defined in \cite[eq. (1.3)]{dantzig}.
%(the choice 1/2 in \ref{deltas}) is arbitrary, we can use any $b<1$).%
%\label{delta_bnd}
%\end{ass}






==> problem_formulation_kfc.tex <==

%\section{Notation and Problem Definition} \label{problem}

\Subsection{Notation}
\label{notation}
%$m$ denotes the signal length while $n$ denotes the number of measurements used at $t>0$.

The set operations $\cup$, $\cap$, and $\setminus$ have the usual meanings. $T^c$ denotes the complement of $T$ w.r.t. $[1,m]:=[1,2,\dots m]$, i.e. $T^c := [1,m] \setminus T$. $|T|$ denotes the size (cardinality) of $T$.%$\phi$ refers to the empty set.

For a vector, $v$, and a set, $T$, $v_T$ denotes the $|T|$ length sub-vector containing the elements of $v$ corresponding to the indices in the set $T$. $\|v\|_k$ denotes the $\ell_k$ norm of a vector $v$. If just $\|v\|$ is used, it refers to $\|v\|_2$. Also, $v_{(i)}$ refers to the $i^{th}$ largest {\em magnitude} element of $v$ (notation taken from \cite{decodinglp}). Thus, for an $m$ length vector, $|v_{(1)}| \ge |v_{(2)}| \dots \ge |v_{(m)}|$.%

We use the notation $v(S)$ to denote the sub-vector of $v$ containing the $S$ smallest magnitude elements of $v$.

For a matrix $M$, $\|M\|_k$ denotes its induced $k$-norm, while just $\|M\|$ refers to $\|M\|_2$. $M'$ denotes the transpose of $M$. For a tall matrix, $M$, $M^\dag : = (M'M)^{-1}M'$.

For a fat matrix $A$, $A_T$ denotes the sub-matrix obtained by extracting the columns of $A$ corresponding to the indices in $T$.
The $S$-restricted isometry constant \cite{decodinglp}, $\delta_S$, for an $n \times m$ matrix (with $n<m$), $A$, is the smallest real number satisfying
\bea
(1- \delta_S) \|c\|^2 \le \|A_T c\|^2 \le (1 + \delta_S) \|c\|^2
\label{def_delta}
\eea
for all subsets $T \subset [1,m]$ of cardinality $|T| \le S$ and all real vectors $c$ of length $|T|$. %It is easy to see that $\|A_T'A_T\| \le (1 + \delta_S)$ and $\|(A_T'A_T)^{-1}\| \le 1/(1- \delta_S)$.
The restricted orthogonality constant \cite{decodinglp}, $\theta_{S,S'}$, is the smallest real number satisfying
\bea
| {c_1}'{A_{T_1}}'A_{T_2} c_2 | \le \theta_{S,S'} \|c_1\| \|c_2\| %\ \text{whenever} \ \|v_1\|_0 \le S  \ \text{and}   \ \|v_2\|_0 \le S'
\label{def_theta}
\eea
for all disjoint sets $T_1, T_2 \subset [1,m]$ with $|T_1| \le S$, $|T_2| \le S'$, $S+S' \le m$, and for all vectors $c_1$, $c_2$ of length $|T_1|$, $|T_2|$.% respectively %By setting $c_1 = {A_{T_1}}'A_{T_2} c_2$ in (\ref{def_theta}), it is easy to see that  $\|{A_{T_1}}'A_{T_2}\| \le \theta_{S,S'}$.

For a square matrix, $Q$, we use $(Q)_{T_1,T_2}$ to denote the sub-matrix of $Q$ containing rows and columns corresponding to the entries in $T_1$ and $T_2$ respectively. $I$ denotes an appropriate sized identity matrix.
{\em The $m \times m$ matrix $I_T$ is defined as}
\bea
(I_T)_{T,T} = I, \ (I_T)_{T^c,[1,m]} = 0, \ (I_T)_{[1,m], T^c} = 0
\label{defI}
\eea
%where $I$ is a $|T|$-identity matrix.
% while  $(I_T)_{T^c,[1,m]} = \mathbf{0}$,  $(I_T)_{[1,m], T^c} = \mathbf{0}$.}




%Let $N_t$ denote the support set of $x_t$, i.e. the set of its non-zero coordinates and let $S_t : = |N_t|$. Let $\hat{N}_t$ denote the estimate of $N_t$. Also, let $\Delta_t$ denote the undetected part of the support at $t$, i.e.  $\Delta_t \defn N_t \setminus \Nhat_{t-1}$ and let $\hat{\Delta}_t$ denote its estimate.% Thus $\Nhat_t = \Nhat_{t-1} \cup \hat{\Delta}_t$.
%$T_t = T_{t-1} \cup \hat{\Delta}_t$.


\Subsection{Problem Definition and Some More Notation}
\label{probdef}
Let $(z_t)_{m \times 1}$ denote the spatial signal at time $t$ and $(y_t)_{n \times 1}$, with $n<m$, denote its noise-corrupted observation vector at $t$, i.e. $y_t = H z_t + w_t$. The signal, $z_t$, is sparse in a given sparsity basis (e.g. wavelet) with orthonormal basis matrix, $\Phi_{m \times m}$, i.e. $x_t \defn \Phi' z_t$ is a sparse vector. We denote its support by $N_t$ and we use $S_t:= |N_t|$ to denote its size. Sparse means that $S_t  \ll  m$. %Here, $H$ is the measurement matrix. %, e.g. a (random $\pm 1$ matrix) i %(e.g. randomly selected rows of a discrete Fourier transform (DFT) matrix in case of MR imaging).  Here $'$ denotes transpose.
Thus the observation model is
\bea
y_t = A x_t + w_t, \ A \defn H \Phi, \ \  \E[w_t]=0, \  \E[w_t w_t']= \sigma^2 I \ \ \ \
 %w_t \sim \n(0,\sigma_{obs}^2 I) %\underbrace{H \Phi}_
\label{obsmod}
\eea
%$H$ is s.t.  (or less) and all $S_t$ column sub-matrices of $A \defn H \Phi$ are ``approximately orthonormal" \cite{dantzig}.  $H$ is the measurement matrix (e.g. randomly selected rows of a Fourier matrix in case of MR imaging).
We assume that $A$ has unit norm columns. The observation noise, $w_t$, is independent identically distributed (i.i.d.) over $t$ and is independent of $x_t$. Our goal is to recursively obtain the best estimates of $x_t$ (or equivalently of the signal, $z_t = \Phi x_t$) using $y_1, \dots y_t$. By {\em recursively}, we mean, use only $y_t$ and the estimate from $t-1$, $\xhat_{t-1}$, to compute the estimate at $t$.

We assume that the sparsity pattern (support) of $x_t$ changes ``slowly" over time. Also the observations are assumed to be incoherent w.r.t. the sparsity basis of the signal, i.e. all $S$-column sub-matrices of $A \defn H \Phi$ are ``approximately orthonormal" (have all nonzero singular values close to 1) \cite{dantzig}, for $S$ a little more than $S_t$. We quantify both the above assumptions after giving the following definition.
%, i.e. $\delta_S = \delta_S(A) < 1$

\bd[Define $\sone$, $\sinf$]
For $A:=H \Phi$, %define the following two quantities:
\ben
\label{deltas}
\item let $\sone$ denote the largest $S$ for which $\delta_S < 1/2$,
\label{delta3s}
\item let $\sinf$ denote the largest $S$ for which $\delta_{2S}+ \theta_{S,2S} < 1$.%\gamma \le
\een
%(the choice 1/2 in \ref{deltas}) is arbitrary, we can use any $b<1$)
\label{delta_bnd}
\ed
\begin{ass}
Assume that
%The following assumptions are used in the entire paper.
%Our algorithm relies on the following.
%In the entire paper, we assume the following. %about $A$ and about sparsity
\ben
\item The additions at any time, $|N_t \setminus N_{t-1}| \le S_a  \ll  S_t$ and the removals, $|N_{t-1} \setminus N_t| \le S_r  \ll  S_t$.% Typically $S_a  \approx S_a$. %Knowledge of $S_a$ or $S_r$ is not needed by the algorithm.%
\item $A$ satisfies $S_t + S_r < \sone$ and $S_a < \sinf$.
\een
\label{initass}
\end{ass}
The slow support change assumption was empirically verified in our recent work \cite{kfcsmri}. We observed that typically $S_a \approx S_r \le S_t/10$, and $S_t$ stays roughly constant. Approximate orthonormality is known to hold with high probability (w.h.p.) when $A$ is a random Gaussian, Rademacher or partial Fourier matrix and $n$ is large enough \cite{decodinglp,dantzig}.
%is approximately orthonormal, i.e.

\subsubsection{More Notation}% (we explain how this is computed later)
We use $\xhat_t$ to denote the estimate of $x_t$ given by our algorithm at time $t$ and $\Nhat_t$ to denote its support estimate. To keep notation simple, we avoid using the subscript $t$ wherever possible. We will use the following sets often.%
\bd[Define $T$, $\Delta$, $\Delta_e$]
We use $T  : = \Nhat_{t-1}$ to denote the support estimate from the previous time. This serves as an initial estimate of the current support.% =T(t)
We use $\Delta := N_t \setminus T$ to denote the unknown part of the support at the current time. % =\Delta(t)
We use $\Delta_e := T \setminus N_t$ to denote the ``erroneous" part of $T$.
\ed
\bd[Define $\tT$, $\tDelta$, $\tDelta_e$]
We use $\tT := \Nhat_t$ to denote the final estimate of the current support.
We use $\tDelta : = N_t \setminus \tT$ to denote the ``misses" in the final estimate and $\tDelta_e := \tT \setminus N_t$ to denote the ``extras". %(extra elements that wrongly got added). (elements of the current support which did not get detected by the algorithm)
\ed

Some more notation - $\xhat_{\CSres}$, $\tDelta_{\dett}$, $\tT_{\dett}$, $\alpha$, $\alpha_{del}$, -  is defined when we give our algorithm in Sec. \ref{lscs}. %(again all of these should have the subscript $t$) $\xhat_{\dett}$, $\Nhat_{\dett}$,



%Assume that the measurement matrix $A:=H \Phi$ satisfies
%\ben
%%\item $\delta_S < \defb < 1$ for all $1 \le S \le \sone$ (e.g. $b=1/2$)
%\label{deltas}
%\item $\delta_S < \defb$ for all $1 \le S \le \sone$,%
%\label{delta3s}
%\item $\delta_{2S}+ \theta_{S,2S} < 1$ for all $1 \le S \le \sinf$ (clearly $\sinf \le \sone$),%
%%\item  $\smax < \sone$ and $\samax < \sinf$.
%\een
%%$\theta_{S,S'}$ is defined in \cite[eq. (1.5)]{dantzig}.
%%$\delta_{\smax + S_{fa}}< 1$. $\delta_S = \delta_S(A)$ is defined in \cite[eq. (1.3)]{dantzig}.
%(the choice 1/2 in \ref{deltas}) is arbitrary, we can use any $b<1$).%
%\label{delta_bnd}
%\end{ass}






==> simulationresults_3.tex <==


%To do: (1) Either remove discussion of LS-CS in the static part or re-run the static simulation with smaller add thresholds and the same del threshold (current one did not use del at all). NOT SO NEEDED: JUST REMOVE LS-CS discussion
%To do: also run the simulation for n=100 when both CS-res and CS similar: NOT NEEDED
%To do: run static simulation with bounded noise and appropriate value of \lambda - MAYBE

%To Do: run STABILITY SIMULATION with deletion at all times AND with  small addition and deletion thresholds.

%To Do: add the random walk simulation also.


\Section{Simulation Results}
\label{sims}
% where a part of the support is known, but the known support may have some error
We discuss three types of simulations in the next three subsections. In the first, we studied a static problem and compared CS-residual error with that of CS. Next we simulated Signal Model \ref{sigmod1} and verified the stability result of Theorem \ref{stabres}. In a third set, we simulated much lower SNRs and compare LS-CS with KF-CS and with LS-CS without deletion. In all our simulations, $A$ was random-Gaussian. We averaged over 100 simulations (noise and signal supports for all times randomly generated in each simulation) for all the time-series simulations and over 50 for the static one.%

%In a final set of three simulations, we compare LS-CS with KF-CS and with LS-CS-without-deletion. With the first set, we demonstrate that whenever the number of deletions becomes significant enough (i.e. for a long enough simulation), LS-CS-without-deletion starts to fail. We also show that when $n$ is large enough so that $A_T'A_T$ remains well-conditioned, and when the rate of addition/deletion is large so that KF-CS does not stabilize between additions/deletions, LS-CS actually outperforms KF-CS. In the second set, we use larger noise and a smaller value of $n$ so that $A_T'A_T$ occasionally becomes ill-conditioned.  This is the situation where KF-CS outperforms LS-CS. Finally we simulate an example of Signal Model \ref{randomwalk}.

%The most important situation where KF-CS is significantly better than LS-CS is when $n$ is smaller ($A_T$ becomes ill-conditioned) and the change of the coefficients over time is slow enough compared to the observation noise. Also note (this we do not plot), if the delay between additions/deletions is small, KF-CS will have slightly smaller error than LS-CS in the stable state (after all/most adds/dels have been detected), while it is not clear which is better just after the addition/deletion time.


\input{table}


\Subsection{Comparing CS-residual with CS}
\label{staticsim}
%In Sec. \ref{csresbound}, we compared the bounds on CS-residual and CS error when $n$ is small. But showing that the CS-residual bound is much smaller only tells us that the performance guarantees for CS-residual are better. It does not necessarily tell us that CS-residual will actually do better than CS. Thus we use simulations to check this.
We simulated a single time instant reconstruction problem (reconstruct $x$ from $y:=Ax+w$) with $m=200$,  $|N|=20$, and with $|\Delta| = 0.1|N|=2=|\Delta_e|$. The noise $w$ was zero mean i.i.d Gaussian. The nonzero signal values, $x_N$, were i.i.d. $\pm 1$ with equal probability.
The sets $N$, $\Delta \subseteq N$ and $\Delta_e  \subseteq N^c$ were uniformly randomly generated each time.
We used four different noise standard deviations ($\sigma = 0.0439*[1,2,4,10]$) and three different choices of $n$ (45, 59, 100).  In Table \ref{static_table}, we compare the normalized MSE of the CS-residual output with that of CS. CS (Dantzig selector) was run with different choices of $\lambda$ while for CS-residual we fixed $\lambda = 4 \sigma$. Except when $n=100$, in all other cases CS-residual outperforms CS significantly. For $n=100$ (large $n$), if $\sigma = 0.04$, CS (with smallest $\lambda$) is better, and if $\sigma = 0.09$, both are similar.
 %This is true even with $n=45$ which is less than even 3 times the support size. With $n=100$, CS is better if noise is small.%CS-residual is better if noise is large.

  %(and hence in future comparisons we only use this).
A few other observations. (1) The best CS error is when we run it with the smallest $\lambda$. Smaller $\lambda$ reduces the size of the feasible set and this encourages more elements of $\xhat$ to be nonzero. When $n$ is small, this is needed for improved error (if $\lambda$ is too large, $\xhat=0$ will be feasible and so it will be the solution). (2) We also compared the CS-residual error with the error of the final LS-CS output (not shown). Only when CS-residual error was small, the support estimation was accurate and in this situation the final LS-CS error was much smaller.%
%(2) We also computed the MSE of Gauss-Dantzig selector and the errors were almost the same as those for Dantzig selector.
%the noise is small enough, the final LS step significantly reduces the error. This is because there is significant reduction in error after the final LS step only when one/both of the additions get detected. When CS-residual error is large, often there will be no detections.%This is true when the detection threshold is set as a fraction of the signal power. We set the detection threshold at $\alpha=0.15*1$. Alternatively if $\alpha$ is set at few times the noise value, then there will be many false detections if CS-residual error is large.
%To do: re-run with smaller add thresholds. Del threshold can be large because the true signal value is at least 2 = 0.5*4 at that time

% ($n=45$ and $\sigma=0.0439$ or $n=59$ and $\sigma \le 0.0878$)  (noise large for a given $n$)

%We used a detection threshold $\alpha = \max(0.15,\sigma)$ and we did not implement the deletion step. The deletion step becomes necessary only for long time series problems when the number of deletions becomes large enough for the matrix $A_T$ to become ill-conditioned because of it.

\input{figures_2}


\Subsection{Verifying LS-CS Stability}
\label{stabsims}
We verified the stability result of Theorem \ref{stabres} in Fig. \ref{stability_fig}. We simulated Signal Model \ref{sigmod1} with $m=200$, $S_0=20$, $S_a=2$ and with $d=8$, $r=2$, $M=3$. Half the $a_i$'s were 0.5, the other half were 0.25. We used $n=59$ and noise was $unif(-c,c)$ with $c=0.0528$. The LS-CS algorithm used  $\lambda=c\|A\|_1=0.35$, $\alpha=c$ and $\alpha_{del}=2.28c$.

In all 100 simulations, the number of misses and extras became exactly zero within $d_0+S_a-1=4$ time units of the addition time, i.e.  the LS-CS estimate became equal to that of the genie-LS. Thus $d_0$ was at most 3 in the simulations. Also, the maximum normalized MSE of LS-CS is 0.3\%.
Compare this to that of CS (Dantzig) with small $\lambda$, which was 30-40\%.
%We also implemented CS (Dantzig) with small $\lambda$, $\lambda=0.035$. Its normalized MSEs were much larger, 30-40\%.
%40-60\% while that of LS-CS was less than 1.2\% at all times, including right before the first new addition got detected. The CS-residual error was slightly higher (less than 2\% at all times), but still much smaller than CS.% $\lambda = 0.3514$ and with

 %A similar approach is used in the COSAMP \cite{cosamp}. %algorithm which is a greedy approach to reconstruct a single sparse signal , and immediately delete


\Subsection{Lower SNR Simulations and Comparing LS-CS and KF-CS}
\label{lowsnrsims}
Next we ran three sets of simulations with much lower signal to noise ratios (SNR). We call them slow-adds-1, slow-adds-2 and fast-adds. In all simulations, $m=200$, $S_0=20$, $S_a=2$ and the noise is $unif(-c,c)$. Also, we used a smaller $\lambda$,  $\lambda = c\|A\|_1/2$ since it encourages more additions.%

We define two quantities: minimum average signal to noise ratio (min-SNR) and  maximum average signal to noise ratio (max-SNR). Min (max) SNR is the ratio of minimum (maximum) average signal magnitude to the noise standard deviation. For $unif(-c,c)$ noise, the standard deviation is $c/\sqrt{3}$. Min-SNR, which occurs right after a new addition, decides how quickly new additions start getting detected (decides $d_0$). Max-SNR decides whether $|\Delta|$ becomes zero before the next addition. Both also depend on $n$ of course.% ($|\Delta|$ is stable or not) quick detection and stability

For the previous subsection (Fig. \ref{stability_fig}), $c/\sqrt{3} = 0.03$.  Minimum average signal magnitude was $(0.5+0.25)/2=0.375$ while maximum was $(M+d\min_i a_i)/2 = (3+8*0.25)/2 = 2.5$. {\em Thus min-SNR was 12.3 while max-SNR was 82.}

In slow-adds-1 (Fig. \ref{kfcs_better_59},  \ref{kfcs_better_59_support}), we use $n=59$, $c=0.1266$ and Signal Model \ref{sigmod1} with $a_i = 0.2$, $M=1$, $d=8$ and $r=3$. Thus {\em min-SNR was $0.2*\sqrt{3}/0.1266 = 2.73$ while max-SNR was $1*\sqrt{3}/0.1266=13.7$ (both are much smaller than 12.3 and 82 respectively)}. Notice the following.
(1) At times when the average misses, $|\tDelta| \neq 0$, LS-CS and KF-CS have similar errors. When average $|\tDelta| = 0$, LS-CS stabilizes to the genie-LS while KF-CS stabilizes to an even smaller MSE value.
(2) Most additions get detected within 2 time units and there are occasionally a few extra additions. This is because we set $\alpha=\alpha_{del}=c/2$ (both very low).
(3) As long as $A_T'A_T$ remains well-conditioned, a few extras do not increase the error visibly above that of the genie-LS. Notice from the plots that even when LS-CS $\approx$ genie-LS, the average extras, $|\tDelta_e|$, are not zero.  (4) The corresponding CS plots (for various $\lambda$'s) are shown in Fig. \ref{CS_kfcs_better_59}. Clearly the errors are much larger.


LS-CS used $\lambda = 0.176$, $\alpha=c/2 =0.06= \alpha_{del}$. Also, it restricted maximum number of additions at a time to $S_a+1$. We also evaluated our assumption that CS at $t=0$ done with large enough $n_0$ finds the support without any error. With $n_0=150$, this was true 90\% of the times, while in other cases there were 1-2 errors. {\em KF-CS was run {\bf with} a deletion step}. It used above parameters and it set $\sigma^2=c^2$, $\sigma_{sys}^2 = 0.01$. For Signal Model \ref{sigmod1}, there are no correct choices of KF parameters. The average of $(x_t-x_{t-1})_i^2$ over $i$ and $t$ was $(0.04*(5/8)*(2/20) + 0.11*(3/8)*(2/20) +0*1*(16/20)) \approx 0.01$ and this motivated the choice of  $\sigma_{sys}^2$. The noise variance is $c^2/3$, but we use a larger value to also model the effect of extra observation error due to the unknown support $\Delta$.%Clearly in this case, the KF in KF-CS is not an optimal estimator.%, it is actually just a linear estimator that uses prior estimates of the non zero coefficient values to improve estimation.
%(0.04*(5/8)*(2/20) + 0.11*(3/8)*(2/20) +0*1*(16/20)=0.0066

In slow-adds-2 (Fig. \ref{kfcs_better_40}, \ref{kfcs_better_40_support}), we kept everything the same, except that we used $n=40$ and $c=0.15$. With such a small $n$, $A_T'A_T$ is more prone to becoming ill-conditioned. If this happens even once, it results in larger error, which in turn results in more extra adds and even worse $A_T'A_T$ at future times. This causes the instability (error increase over time) of LS-CS. KF-CS is more robust to occasional ill-conditioning of $A_T'A_T$, since it never inverts this matrix and since it uses past signal estimates.%since it uses prior signal estimates.%and so its error remains roughly stable.  uses the prior model and

In fast-adds (Fig. \ref{fast_adds_dels}, \ref{fast_adds_dels_support}), we use $n=59$, $c=0.0528$ and a slightly modified Signal Model \ref{sigmod1} with $a_i = 0.2$, $M=1$, $d=3$ and $r=2$. Thus {\em min SNR was $0.2*\sqrt{3}/0.0528 = 6.6$ while max SNR was $0.6*\sqrt{3}/0.0528= 19.7$.} Both are smaller than the stability simulation, but larger than the slow-adds simulations. This was needed because in this case the delay between addition times was only 3, and so quick detection was needed to ensure error stability. Because of the small value of $d$, KF-CS never gets a chance to stabilize. Its errors are larger than LS-CS at new addition times. Also, clearly LS-CS-without-deletion is unstable.
LS-CS used $\lambda = 0.176$, $\alpha=c = 0.05 = \alpha_{del}$ and maximum additions per unit time of $S_a=2$. KF-CS used all this and $\sigma^2=c^2$,  $\sigma_{sys}^2 = 0.01$. %CS at $t=0$ was not run.


%Finally, Fig. \ref{oldsim} simulates the random walk model with increasing support (Signal Model \ref{randomwalk}) with $m=256$, $S_0=8$, $S_a=2$, $d=5$, $\smax = 26$ and $\sigma_{sys}=1$. Measurements used $n=n_0=72$ and Gaussian noise with $\sigma=0.16$.% Notice that KF-CS gets to within a small error of the genie-KF

%In a final set of three simulations, we compare LS-CS with KF-CS and with LS-CS-without-deletion. With the first set, we demonstrate that whenever the number of deletions becomes significant enough (i.e. for a long enough simulation), LS-CS-without-deletion starts to fail. We also show that when $n$ is large enough so that $A_T'A_T$ remains well-conditioned, and when the rate of addition/deletion is large so that KF-CS does not stabilize between additions/deletions, LS-CS actually outperforms KF-CS. In the second set, we use larger noise and a smaller value of $n$ so that $A_T'A_T$ occasionally becomes ill-conditioned.  This is the situation where KF-CS outperforms LS-CS. Finally we simulate an example of Signal Model \ref{randomwalk}.

\subsubsection{Setting $\alpha, \alpha_{del}$} % average
\label{setthresh}
The thumb rule from literature is to set $\alpha$ at roughly the noise level \cite{dantzig}. So we set it somewhere between $c/2$ and $c$. %this is $c/1.732$ and so we set $\alpha=c/2$.
Usually the error after the second LS step (error of $\xhat_{t,\dett}$) is lower than that of CS-residual. If min-SNR is high enough, even if we set $\alpha_{del}$ at a higher value, there will be no false deletions and it may help to reduce/remove the extras almost immediately. This was done in the stability simulation.

But if min-SNR is not high enough or if $d$ is smaller, this argument may not work. In this case, we suggest $\alpha_{del}=\alpha$. With this, there may be a few more extras, but usually, the error increase due to a few extras is negligible, while that due to even one miss is significant (see Fig. \ref{kfcs_better_59},  \ref{kfcs_better_59_support}).%due to even one miss is much larger than the error false additions and removed coefficients

%Typically the error after the second LS step is lower than that of CS-residual. If min-SNR is high enough (as in the stability simulation), even if we set $ \alpha_{del}$ higher, there will be no false deletions, but it will help to almost immediately delete the extras. But if min-SNR is not high enough and/or if $d$ is small, this argument will not work and it is better to set $\alpha_{del}=\alpha$. This is because the error increase due to a few extras is usually negligible, but that due to even one miss is significant.%due to even one miss is much larger than the error false additions and removed coefficients


\Section{Conclusions}
\label{conclusions}
We formulated the problem of recursive reconstruction of sparse signal sequences from noisy observations as one of noisy CS with partly known support (the support estimate from the previous time serves as the ``known" part). Our proposed solution, LS CS-residual (LS-CS), replaces CS on the raw observation by CS on the LS residual, computed using the known part of the support. %Kalman Filtered CS (KF-CS), which replaces the LS residual by the KF residual, is also briefly introduced. % (resp. KF)
We obtained bounds on CS-residual error that hold if the ``error", $\Delta_e$, in the known part of the support, $T$, is small enough (so that $|T| \le \sone$). The bound is small if the size of the unknown support, $\Delta$, is also small compared to that of the true support, $N$.
When the number of available measurements, $n$, is small, we showed that our bound is much smaller than the CS error bound if $|\Delta|, |\Delta_e|$ are small enough.
We used this bound to show the stability of LS-CS over time for a simple signal model of signal increase/decrease. By ``stability" we mean that $|\Delta|, |\Delta_e|$ remain bounded by small values compared to the support size. Extensive simulation results backing our claims are shown.%

%We also showed that they become zero within a finite delay of a new addition time.  % (the LS-CS estimate becomes equal to the genie-LS estimate)
%KF-CS stability is studied in the Supplementary Material.
%A weaker result was given for KF-CS under a zero-drift random-walk model.% before the next addition time

%It was shown that if the noise is bounded and the number of measurements, $n$, is enough for certain $\delta_S$'s and $\theta_{S,S'}$'s to be small enough; and if the delay between addition times is large enough compared to the rate of magnitude increase of new additions, then ``stability" is ensured, i.e. $|\Delta|$, $|T|$ remain bounded and  $|\Delta|$ goes to zero within a finite delay of a new set of additions.

An open question is how to prove stability for a stochastic signal model that (a) uses a random walk model with drift given by the current model for coefficient increase/decrease, (b) uses a stationary model for ``constant" coefficients, and (c) that assumes a statistical prior on support change, e.g. a modification of the model of \cite{schniter} can be used. %This will be needed to study KF-CS stability under this model. %signal-dependent and adds random jitter to the addition/removal times
Finally, in this work, we did not study exact reconstruction using much fewer noise-free measurements. We are doing this in  \cite{isitmodcs,icipmodcs}.% for the currently nonzero coefficients  when part of the support is known magnitude increase/decrease


%. This will be needed for analyzing KF-CS stability under the above fully Bayesian model.




%The difference from Signal Model \ref{sigmod1} was that decrease/removals occurred during $[t_j+1, t_j+r]$ instead of $[t_{j+1}-r,t_{j+1}-1]$, i.e. removal coefficients were decreasing at the same time that newly added coefficients were increasing.



%\Subsection{Lower SNR Simulations and Comparing LS-CS and KF-CS}
%Next, we ran two sets of simulations for much lower signal to noise ratios (SNR). %and for faster addition/deletion or lower $n$.
%
%
%Thus minimum SNR was $a_i/c = 0.2/0.05 = 4$, while maximum SNR was $d a_i /c = 12$. Compare this with the previous subsection where average minimum SNR was average $a_i/c = 0.375/0.05 = 7.5$, while average maximum SNR was $2.5/0.05 = 50$.
%$n=59$, $d=8, r=3, M=1, a_i=0.2$: minimum SNR was $a_i/c = 0.2/0.1266 = 1.6$ and maximum SNR was $M/c = 1/0.1266 = 7.9$. Minimum SNR decides how quickly all additions get detected, maximum decides whether they will all get detected before next addition time, thus max SNR ensures stability, while minimum SNR decides the maximum error bound
%
%
%%more difficult scenarios - faster additions/deletions and smaller $n$. In both cases, the SNR as well as the rate of increase of new addition magnitudes was also smaller than in the previous subsection.
%
%For the first set of simulations, we simulated a time series of $x_t$ with $a_i = 0.2$ for all new additions, $M=1$, $d=3$ (this means the maximum value of new additions was only 0.6) and $r=2$. The one difference from Signal Model \ref{sigmod1} was that removals occurred at $t_j+r$ instead of $t_{j+1}-r$, i.e. removal coefficients were decreasing at the same time that newly added coefficients were increasing.
%We used $m=200$, $S_1=20$ and $S_a = 2$, $n=59$ and the noise was still i.i.d. $unif(-c,c)$ with $c=0.0528$. The coefficients that existed at $t=1$ were $\pm M$. In this case the performance of LS-CS and KF-CS was similar with LS-CS outperforming KF-CS at the new addition times and a little after. We also compared LS-CS with LS-CS-without-deletion which starts to fail whenever enough deletions have occurred (since $A_T$ becomes ill-conditioned).
%
%In this simulation, we used  a smaller $\lambda$ in the CS-residual step of LS-CS ($\lambda = 0.176$ instead of  $\lambda = 0.35$) since it encourages more additions. Also, we used $\alpha = \alpha_{del}=0.0528$. Notice that the threshold should be at least equal to 1-2 times the average noise level $c/\sqrt{3}$, because even with the least squared error estimator anything smaller than that will not get estimated correctly. We used $1.732*c/\sqrt{3}=c$.
%The KF-CS implementation used all of the above. Also, the KF used $\sigma^2 = c$ and  $\sigma_{sys}^2 = 0.1$. For the signal model that we use there are no correct choices of KF parameters. In this simulation, a new addition increases at rate $a_i=0.2$ and a coefficient in the ``starting to get removed" phase decreases at an average rate of 0.3. At every $r=2$ out of $d=3$ time units, there  are 2 coefficients increasing, 2 decreasing, the other 18 are constant, while at 1 out of 3 time units (the addition times), there are only 2 coefficients increasing.
%Thus the average of $(x_t-x_{t-1})_i^2$ over space and time is is $(0.04*(2/22)*1 + 0.09*2*(2/3)*(2/22) + 0*(18/22)*(1/3) \approx 0.01$. Based on this heuristic we use $\sigma_{sys}^2 = 0.01$.
%The observation noise variance is $c^2/3$, but we instead use a larger value of $c^2$ which also models the extra error due to the unknown part of the support $\Delta$. The KF in KF-CS is no longer the optimal filter, it is actually just a linear estimator that uses prior estimates of the non zero coefficient values to improve estimation.
%%Also, at the time instant after a new addition $\sigma_{sys}$ for that coefficient was replaced by a higher $\sigma_{init} = 0.5$
%%To do for KF: use max(a_i), c^2/3, and no sigma_init
%
%In a second simulation, we simulated a time series of $x_t$ using the signal model of ? with $a_i = 0.2$ for all new additions, $M=1$, $d=8$ and $r=3$. We used only $n=40$ observations and larger observation noise - i.i.d $unif(-c,c)$ with $c=0.1266$. The rest was the same as earlier $m=200$, $S_1=20$, $S_a=2$. Since $n$ was much smaller, and observation noise was larger, KF-CS significantly outperformed LS-CS. Because $n$ is so small, $A_T$ starts to become ill-conditioned with even one or two false additions and this amplifies the effect of noise (which is also larger). Thus LS-CS error becomes unstable. But because of the prior knowledge used by the KF in KF-CS, this does not happen.
%
%


%%Addition/deletion thresholds were also set much lower, we set them at the maximum noise level, i.e. we used $\alpha = \alpha_{del}=0.0528$.


==> simulations8.tex <==
%%\clearpage
%
%\begin{figure*}[ht!]
%\centerline{
%\subfigure{
%\label{sims_nodel}
%\psfig{file = C:/Code/KFCS/data_kfcs4_cs.eps, height = 3cm,width=5cm}
%}
%\subfigure{
%\label{sims_del}
%\psfig{file = C:/Code/KFCS/data3_kfcs4_cs.eps, height = 3cm,width=5cm} %width=4cm,
%}
%}
%\vspace{-0.15in}
%\caption{{\small MSE plots of KF-CS compared against regular CS and against Genie-Aided KF which serves as the benchmark. In Fig. \ref{sims_nodel}, large KF-CS error occurs at and after $t=10, 20, 30$, when new additions occur. But once the addition is detected, it gradually reduces to that of GA-KF (or slightly higher). CS error is much larger, maximum value is 45. In Fig. \ref{sims_del}, again similar trend is observed. But CS error is much larger beyond $t=50$ when $S_t \ge 26$. Maximum CS error was 425.
%%In Fig. \ref{sims_del}, the largest KF-CS error occurs at $t=51 = t_{a,max}$. Also note that in this case beyond $t \approx 43$ (when $S_t = 19$ and keeps increasing to $S_{max}=25$), the CS error is very large.
%}}
%\label{fig}
%\end{figure*}


% and we simulated Gaussian noise (not truncated)
\section{Simulation Results}
\label{sims}
%The sparsity sizes $S_t = |N_t|$.
We simulated a time sequence of sparse $m=256$ length signals, $z_t = x_t$ which follow (\ref{sysmod}) with $\sigma_{sys}^2=1$ and support sets, $N_{t-1} \subseteq N_t$.
We started with an initial sparsity size, $S_1=|N_1|=8$ and for $10 \le t \le 50$, we added 2 new elements to $N_t$ every 5 time units. Thus $\smax=26 = S_t, \forall \ t \ge 50$. The measurement matrix, $A = H$ was simulated as in \cite{dantzig} by generating $n \times m$ i.i.d. Gaussian entries, with $n=72$, and normalizing each column of the resulting matrix. The observation noise was a zero mean i.i.d. Gaussian with variance was $\sigma_{obs}^2 = ( (1/3)\sqrt{16/n})^2$ (this is taken from \cite{dantzig}).
%Notice that $26 > n/3 = 24$ and thus $\delta_{3\smax}$ cannot be smaller than 1. As a result, the number of measurements becomes too small for CS to work.%, i.e. Theorem 1.1 of \cite{dantzig} will not apply

%, $\alpha_{fe} = 2n$, $\alpha_{z} = \sigma_{obs}^2$, $k = 5$, $k' = 3$.
%somewhere between $0.7n/\log_2 m \approx 6$ and $(1.25n/\log_2 m) \approx 11$
We implemented LS-CS-res-LS and KF-CS-res-LS with and without the deletion step given in Algorithm \ref{kfcs}. We also implemented KF-CS-res-KF.
The parameters used were $\lambda_m = \sqrt{2 \log_2 m}=4$ and $\alpha = 9 \sigma_{obs}^2$. For the deletion step, we used $\alpha_{z} = \sigma_{obs}^2$, $k = 5$, $k' = 3$.
Since the observation noise is not truncated, occasionally the addition step can result in a very large number of false additions. To prevent this, we restricted the maximum number of allowed additions at any time to $cn/\log_2 m$ ($c$ between 0.7 and 1.25) largest magnitude coefficients. Also, we reduced the number of additions to $\Nhat_t$ when $A_{\Nhat_t}$ became rank deficient (we kept removing the smallest added coefficients until $A_{\Nhat_t}$ became full rank).%Thirdly, for KF-CS-res-KF, we set $\sigma_{init}^2 = 3 \sigma_{sys}^2$ ($\sigma_{init}^2$ is used instead of $\sigma_{sys}^2$ the first time a new coefficient gets added). This was done because typically an addition about 3 time instants to get detected.


We simulated the system described above 100 times and compared the normalized MSE (MSE normalized by mean signal energy) of LS-CS-res-LS and KF-CS-res-LS with that of genie-aided KF and of simple CS (followed by thresholding and least squares estimation as in Gauss-Dantzig \cite{dantzig}).
When $S_t$ was anything larger than 8 or 9 ($\approx n/\log_2 m$), the Gauss-Dantzig selector gave very large error (MSE of the order of $10^8$), while solving noiseless CS ($\min ||\beta||_1,  s.t. A \beta = y_t$) followed by thresholding and LS gave much smaller errors. Hence we show plots of the latter in Fig. \ref{CScompare}. Notice that for $t \ge 50$, $S_t = 26 > n/3 = 24$ and thus $\delta_{3\smax}$ cannot be smaller than 1.  As a result, the number of measurements becomes too small for CS to work. In fact, as can be seen from the plot, for $S_t=20$ or more ($t \ge 35$), the CS error is {\em much larger} than that of either LS-CS-res-LS or KF-CS-res-LS. As an aside note that if we look at the MSE plot of CS (we show only normalized MSE plots), it does increase linearly with $t$, while that of LS-CS-res-LS or KF-CS-res-LS remains small, i.e. their difference increases linearly with $t$.
% Also, the final LS step in LS-CS-res-LS greatly improves the MSE compared to LS-CS-res, especially when $|\Delta|$ is large, i.e. at a new addition time or a little after that.

 %, i.e. Theorem 1.1 of \cite{dantzig} will not apply

In Fig. \ref{algos_compare}, we compare LS-CS-res-LS with KF-CS-res-LS, KF-CS-res-KF and genie-aided KF. In Fig. \ref{deletion_compare}, we compare KF-CS-res-LS with and without the deletion step. The following observations can be made.
(a) When all additions are not detected, nothing much can be said about LS-CS-res-LS versus KF-CS-res-LS since the KF is being run with wrong model parameters. But, when w.h.p. all additions have been detected and the KF has stabilized, i.e. roughly after $t=55$,  KF-CS-res-LS outperforms LS-CS-res-LS. This follows because when all additions are detected and the KF stabilizes, it stabilizes to the KF with correct model parameters (genie-aided KF) which will always outperform the genie-aided LS. %LS with correct model parameters (
(b) Even though all assumptions of Theorem \ref{thm_conv} are not satisfied (noise is not truncated and number of false additions is only small not zero), KF-CS-res-LS does approach the genie-aided KF for $t$ large.
(c) Replacing the final LS step by a KF (KF-CS-res-KF) does not help much.
(d) The deletion step improves performance most of the time. Notice that in the current work, we did not experiment with many choices of the threshold or with the maximum allowed additions. As we show in \cite{kfcsmri}, if this is carefully done, the deletion step can be more useful.

In Fig. \ref{mean_fa}, we plot the mean number of false additions, $\Nhat_{t-1} \setminus N_t$,  for LS-CS-res-LS and KF-CS-res-LS. As can be seen, this number is less than 2, i.e. is small compared to $S_t$. %So the assumption of $S_{fa}$ being small, used in Theorems \ref{thm1} and \ref{thm2}, is valid.
In Fig. \ref{mean_misses}, we plot the mean $N_t \setminus \Nhat_t$. The mean is between 0.3-0.4 before a new addition, which means that most of the times, a set of additions does get detected before a new one.%

In a second set of simulations, we started with $S_1=8$ and then for $10 \le t \le 30$, we added 4 new elements every 10 time units. Thus $\smax=20 = S_t, \forall \ t \ge 30$. Everything else was the same as above. We  compare CS with LS-CS-res-LS, KF-CS-res-LS in Fig. \ref{model2}. Here at the initial time instants, when $S_t$ is small, CS actually outperforms CS-res. Also, for larger $t$ the difference in performance is not as drastic, since $\smax=20$. The mean of  $N_t \setminus \Nhat_t$ for LS-CS-res-LS/KF-CS-res-LS before a new addition was only about 0.1 in this case (since delay between addition times was larger).%


%%The truncated noise assumption is not valid but in spite of that the error of LS-CS-res-LS is much smaller than that of CS.
%
%
%
%%Noiseless CS was used instead of Dantzig selector since it gave much lower errors.%Note that when $S$ was anything larger than 8 or 9 ($\approx n/\log_2 m$), the Gauss-Dantzig selector gave very large error (MSE of the order of $10^8$), while solving noiseless CS ($\min ||\beta||_1,  s.t. A \beta = y_t$) followed by thresholding and LS gave much smaller errors. Hence we show plots of the latter in Fig. \ref{sims_nodel}. to get the final estimate
%
%% and if the observation noise is bounded support (e.g. truncated Gaussian)
%Lemma \ref{nofalseadd_thm11bnd} says that if the addition threshold was set high enough ($\alpha_a = B_1$ where $B_1$ is the CS error upper bound), then there would be no false additions. But if we set the addition threshold very high, then for the initial time instants, the KF-CS estimation error would be large and it will do worse than regular CS. Thus, in practice, we set $\alpha_a$ lower, but we implement the false addition detection and removal scheme described in Sec. \ref{kfcswithdel}.
%We evaluated its performance using the following set of simulations. We simulated a time sequence of sparse $m$=256 length signals, $z_t = x_t$ which follow (\ref{sysmod}) with $\sigma_{sys}^2=1$ and nonzero sets, $N_{t-1} \subseteq N_t, \ \forall t$ satisfying $N_t = N_1, \forall t < 10$, $N_t = N_{10}, \forall 10 \le t < 20$,  $N_t = N_{20}, \forall 20 \le t < 30$, $N_t = N_{30}, \forall 30 \le t < 100$ and $|N_1| = 8$,  $|N_{10}| = 12$, $|N_{20}| = 16$, $|N_{30}| = 20$. Thus $S_{max}=20$. The set $N_1$ and all the additions were generated uniformly at random from the remaining elements out of $[1:m]$. The measurement matrix, $A = H$ was simulated as in \cite{dantzig} by generating $n \times m$ i.i.d. Gaussian entries (with $n=72$) and normalizing each column of the resulting matrix. The observation noise variance was $\sigma_{obs}^2 = ( (1/3)\sqrt{16/n})^2$ (this is taken from \cite{dantzig}) and we simulated Gaussian noise (not truncated).
%
%%There were some false additions occasionally, most of which eventually got removed. But   %given in Algorithm \ref{kfcsdel}
%We implemented KF-CS with $\lambda_m = \sqrt{2 \log_2 m}=4$, $\alpha_a = 9 \sigma_{obs}^2$, $\alpha_{fe} = 2n$, $\alpha_{z} = \sigma_{obs}^2$, $k = 5$, $k' = 3$. Since the observation noise was not truncated, occasionally the addition step resulted in a very large number of false additions, which made $A_{T_t}'A_{T_t}$ singular (or almost singular) resulting in large errors at all future $t$. To prevent this, we set a maximum value for the number of allowed additions: we allowed at most $(1.25n/\log_2 m)$ largest magnitude coefficient estimates larger than $\alpha_a$ to be added. Also, typically an addition took 2-3 time instants to get detected. Thus we set $\sigma_{init}^2 = 3 \sigma_{sys}^2$ ($\sigma_{init}^2$ is used instead of $\sigma_{sys}^2$ the first time a new coefficient gets added).
%We simulated the above system 100 times and compared the MSE of KF-CS with that of GA-KF and of regular CS (followed by thresholding and least squares estimation as in Gauss-Dantzig \cite{dantzig}). %Noiseless CS was used instead of DS since it gave much lower errors.%Note that when $S$ was anything larger than 8 or 9 ($\approx n/\log_2 m$), the Gauss-Dantzig selector gave very large error (MSE of the order of $10^8$), while solving noiseless CS ($\min ||\beta||_1,  s.t. A \beta = y_t$) followed by thresholding and LS gave much smaller errors. Hence we show plots of the latter in Fig. \ref{sims_nodel}. to get the final estimate
%
%In a second set of simulations, shown in Fig. \ref{sims_del}, we started with $S_1=8$ and for $10 \le t \le 50$, we added 2 new elements every 5 time units. Thus $S_{max}=26 = S_t, \forall \ t \ge 50$. Note $26 > n/3 = 24$ and thus $\delta_{3S_{max}}$ cannot be smaller than 1, i.e. Theorem 1.1 of \cite{dantzig} will not apply. This resulted in much larger errors in regular CS as compared to the first set of simulations.% But KF-CS came close to the GA-KF error sometime after $t=50$. This is because KF-CS has to add at most $\max_t |\Delta_t|$ (which is usually much smaller than $S_{max}$) new coefficients at any time.%


==> simulations8_mod.tex <==
%%\clearpage
%
%\begin{figure*}[ht!]
%\centerline{
%\subfigure{
%\label{sims_nodel}
%\psfig{file = C:/Code/KFCS/data_kfcs4_cs.eps, height = 3cm,width=5cm}
%}
%\subfigure{
%\label{sims_del}
%\psfig{file = C:/Code/KFCS/data3_kfcs4_cs.eps, height = 3cm,width=5cm} %width=4cm,
%}
%}
%\vspace{-0.15in}
%\caption{{\small MSE plots of KF-CS compared against regular CS and against Genie-Aided KF which serves as the benchmark. In Fig. \ref{sims_nodel}, large KF-CS error occurs at and after $t=10, 20, 30$, when new additions occur. But once the addition is detected, it gradually reduces to that of GA-KF (or slightly higher). CS error is much larger, maximum value is 45. In Fig. \ref{sims_del}, again similar trend is observed. But CS error is much larger beyond $t=50$ when $S_t \ge 26$. Maximum CS error was 425.
%%In Fig. \ref{sims_del}, the largest KF-CS error occurs at $t=51 = t_{a,max}$. Also note that in this case beyond $t \approx 43$ (when $S_t = 19$ and keeps increasing to $S_{max}=25$), the CS error is very large.
%}}
%\label{fig}
%\end{figure*}

\input{figs8}


% and we simulated Gaussian noise (not truncated)
\section{Simulation Results}
\label{sims}
%The sparsity sizes $S_t = |N_t|$.
We simulated a time sequence of sparse $m=256$ length signals, $z_t = x_t$ which follow (\ref{sysmod}) with $\sigma_{sys}^2=1$ and support sets, $N_{t-1} \subseteq N_t$.
We started with an initial sparsity size, $S_1=|N_1|=8$ and for $10 \le t \le 50$, we added 2 new elements to $N_t$ every 5 time units. Thus $\smax=26 = S_t, \forall \ t \ge 50$. The measurement matrix, $A = H$ was simulated as in \cite{dantzig} by generating $n \times m$ i.i.d. Gaussian entries, with $n=72$, and normalizing each column of the resulting matrix. The observation noise was a zero mean i.i.d. Gaussian (we did not use bounded noise for simulations) with variance was $\sigma_{obs}^2 = ( (1/3)\sqrt{16/n})^2$ (this is taken from \cite{dantzig}).
%Notice that $26 > n/3 = 24$ and thus $\delta_{3\smax}$ cannot be smaller than 1. As a result, the number of measurements becomes too small for CS to work.%, i.e. Theorem 1.1 of \cite{dantzig} will not apply

%, $\alpha_{fe} = 2n$, $\alpha_{z} = \sigma_{obs}^2$, $k = 5$, $k' = 3$.
%somewhere between $0.7n/\log_2 m \approx 6$ and $(1.25n/\log_2 m) \approx 11$
We implemented LS-CS-res-LS and KF-CS-res-LS with and without the deletion step given in Algorithm \ref{kfcs}. We also implemented KF-CS-res-KF.
The parameters used were $\lambda = \sqrt{2 \log_2 m} \sigma_{obs} = 4 \sigma_{obs}$ and $\alpha = 9 \sigma_{obs}^2$. For the deletion step, we used $\alpha_{z} = \sigma_{obs}^2$, $k = 5$, $k' = 3$.
Since the observation noise is not truncated, occasionally the addition step can result in a very large number of false additions. To prevent this, we restricted the maximum number of allowed additions at any time to $cn/\log_2 m$ ($c$ between 0.7 and 1.25) largest magnitude coefficients. Also, we reduced the number of additions to $\Nhat_t$ when $A_{\Nhat_t}$ became rank deficient (we kept removing the smallest added coefficients until $A_{\Nhat_t}$ became full rank).%Thirdly, for KF-CS-res-KF, we set $\sigma_{init}^2 = 3 \sigma_{sys}^2$ ($\sigma_{init}^2$ is used instead of $\sigma_{sys}^2$ the first time a new coefficient gets added). This was done because typically an addition about 3 time instants to get detected.

% (MSE normalized by mean signal power)
We simulated the system described above 100 times and compared the normalized MSE of LS-CS-res-LS and KF-CS-res-LS with that of genie-aided KF and of simple CS (followed by thresholding and least squares estimation as in Gauss-Dantzig \cite{dantzig}).
When $S_t$ was anything larger than 8 or 9 ($\approx n/\log_2 m$), the Gauss-Dantzig selector gave very large error (MSE of the order of $10^8$), while solving noiseless CS ($\min ||\beta||_1,  s.t. A \beta = y_t$) followed by thresholding and LS gave much smaller errors. Hence we show plots of the latter in Fig. \ref{CScompare}. Notice that for $t \ge 50$, $S_t = 26 > n/3 = 24$ and thus $\delta_{3\smax}$ cannot be smaller than 1.  As a result, the number of measurements becomes too small for CS to work. In fact, as can be seen from the plot, for $S_t=20$ or more ($t \ge 35$), the CS error is {\em much larger} than that of either LS-CS-res-LS or KF-CS-res-LS. As an aside note that if we look at the MSE plot of CS (we show only normalized MSE plots), it does increase linearly with $t$, while that of LS-CS-res-LS or KF-CS-res-LS remains small and bounded, i.e. their difference increases linearly with $t$. The MSE plots are compared in \cite{kfcspap}.
% Also, the final LS step in LS-CS-res-LS greatly improves the MSE compared to LS-CS-res, especially when $|\Delta|$ is large, i.e. at a new addition time or a little after that.

 %, i.e. Theorem 1.1 of \cite{dantzig} will not apply

In Fig. \ref{algos_compare}, we compare LS-CS-res-LS with KF-CS-res-LS, KF-CS-res-KF and genie-aided KF. In Fig. \ref{deletion_compare}, we compare KF-CS-res-LS with and without the deletion step. The following observations can be made.
(a) When all additions are not detected, nothing much can be said about LS-CS-res-LS versus KF-CS-res-LS since the KF is being run with wrong model parameters. But, when w.h.p. all additions have been detected and the KF has stabilized, i.e. roughly after $t=55$,  KF-CS-res-LS outperforms LS-CS-res-LS. This follows because when all additions are detected and the KF stabilizes, it stabilizes to the KF with correct model parameters (genie-aided KF) which will always outperform the genie-aided LS. %LS with correct model parameters (
(b) Even though all assumptions of Theorem \ref{thm_conv} are not satisfied (noise is not bounded and number of false additions is only small not zero), KF-CS-res-LS does approach the genie-aided KF for $t$ large.
(c) Replacing the final LS step by a KF (KF-CS-res-KF) does not help much.
(d) The deletion step improves performance most of the time. Notice that in the current work, we did not experiment with many choices of the threshold or with the maximum allowed additions. As we show in \cite{kfcsmri}, if this is carefully done, the deletion step can be more useful.

In Fig. \ref{mean_fa}, we plot the mean number of false additions, $\Nhat_{t-1} \setminus N_t$,  for LS-CS-res-LS and KF-CS-res-LS. As can be seen, this number is less than 2, i.e. is small compared to $S_t$. %So the assumption of $S_{fa}$ being small, used in Theorems \ref{thm1} and \ref{thm2}, is valid.
In Fig. \ref{mean_misses}, we plot the mean $N_t \setminus \Nhat_t$. The mean is between 0.3-0.4 before a new addition, which means that most of the times, a set of additions does get detected before a new one.%

In a second set of simulations, we started with $S_1=8$ and then for $10 \le t \le 30$, we added 4 new elements every 10 time units. Thus $\smax=20 = S_t, \forall \ t \ge 30$. Everything else was the same as above. We  compare CS with LS-CS-res-LS, KF-CS-res-LS in Fig. \ref{model2}. Here at the initial time instants, when $S_t$ is small, CS actually outperforms CS-res. Also, for larger $t$ the difference in performance is not as drastic, since $\smax=20$. The mean of  $N_t \setminus \Nhat_t$ for LS-CS-res-LS/KF-CS-res-LS before a new addition was only about 0.1 in this case (since delay between addition times was larger).%


%%The truncated noise assumption is not valid but in spite of that the error of LS-CS-res-LS is much smaller than that of CS.
%
%
%
%%Noiseless CS was used instead of Dantzig selector since it gave much lower errors.%Note that when $S$ was anything larger than 8 or 9 ($\approx n/\log_2 m$), the Gauss-Dantzig selector gave very large error (MSE of the order of $10^8$), while solving noiseless CS ($\min ||\beta||_1,  s.t. A \beta = y_t$) followed by thresholding and LS gave much smaller errors. Hence we show plots of the latter in Fig. \ref{sims_nodel}. to get the final estimate
%
%% and if the observation noise is bounded support (e.g. truncated Gaussian)
%Lemma \ref{nofalseadd_thm11bnd} says that if the addition threshold was set high enough ($\alpha_a = B_1$ where $B_1$ is the CS error upper bound), then there would be no false additions. But if we set the addition threshold very high, then for the initial time instants, the KF-CS estimation error would be large and it will do worse than regular CS. Thus, in practice, we set $\alpha_a$ lower, but we implement the false addition detection and removal scheme described in Sec. \ref{kfcswithdel}.
%We evaluated its performance using the following set of simulations. We simulated a time sequence of sparse $m$=256 length signals, $z_t = x_t$ which follow (\ref{sysmod}) with $\sigma_{sys}^2=1$ and nonzero sets, $N_{t-1} \subseteq N_t, \ \forall t$ satisfying $N_t = N_1, \forall t < 10$, $N_t = N_{10}, \forall 10 \le t < 20$,  $N_t = N_{20}, \forall 20 \le t < 30$, $N_t = N_{30}, \forall 30 \le t < 100$ and $|N_1| = 8$,  $|N_{10}| = 12$, $|N_{20}| = 16$, $|N_{30}| = 20$. Thus $S_{max}=20$. The set $N_1$ and all the additions were generated uniformly at random from the remaining elements out of $[1:m]$. The measurement matrix, $A = H$ was simulated as in \cite{dantzig} by generating $n \times m$ i.i.d. Gaussian entries (with $n=72$) and normalizing each column of the resulting matrix. The observation noise variance was $\sigma_{obs}^2 = ( (1/3)\sqrt{16/n})^2$ (this is taken from \cite{dantzig}) and we simulated Gaussian noise (not truncated).
%
%%There were some false additions occasionally, most of which eventually got removed. But   %given in Algorithm \ref{kfcsdel}
%We implemented KF-CS with $\lambda_m = \sqrt{2 \log_2 m}=4$, $\alpha_a = 9 \sigma_{obs}^2$, $\alpha_{fe} = 2n$, $\alpha_{z} = \sigma_{obs}^2$, $k = 5$, $k' = 3$. Since the observation noise was not truncated, occasionally the addition step resulted in a very large number of false additions, which made $A_{T_t}'A_{T_t}$ singular (or almost singular) resulting in large errors at all future $t$. To prevent this, we set a maximum value for the number of allowed additions: we allowed at most $(1.25n/\log_2 m)$ largest magnitude coefficient estimates larger than $\alpha_a$ to be added. Also, typically an addition took 2-3 time instants to get detected. Thus we set $\sigma_{init}^2 = 3 \sigma_{sys}^2$ ($\sigma_{init}^2$ is used instead of $\sigma_{sys}^2$ the first time a new coefficient gets added).
%We simulated the above system 100 times and compared the MSE of KF-CS with that of GA-KF and of regular CS (followed by thresholding and least squares estimation as in Gauss-Dantzig \cite{dantzig}). %Noiseless CS was used instead of DS since it gave much lower errors.%Note that when $S$ was anything larger than 8 or 9 ($\approx n/\log_2 m$), the Gauss-Dantzig selector gave very large error (MSE of the order of $10^8$), while solving noiseless CS ($\min ||\beta||_1,  s.t. A \beta = y_t$) followed by thresholding and LS gave much smaller errors. Hence we show plots of the latter in Fig. \ref{sims_nodel}. to get the final estimate
%
%In a second set of simulations, shown in Fig. \ref{sims_del}, we started with $S_1=8$ and for $10 \le t \le 50$, we added 2 new elements every 5 time units. Thus $S_{max}=26 = S_t, \forall \ t \ge 50$. Note $26 > n/3 = 24$ and thus $\delta_{3S_{max}}$ cannot be smaller than 1, i.e. Theorem 1.1 of \cite{dantzig} will not apply. This resulted in much larger errors in regular CS as compared to the first set of simulations.% But KF-CS came close to the GA-KF error sometime after $t=50$. This is because KF-CS has to add at most $\max_t |\Delta_t|$ (which is usually much smaller than $S_{max}$) new coefficients at any time.%


==> stability_kfcs_2.tex <==

\section{Kalman Filtered CS-residual*}% to improve the accuracy of simple CS
\label{kfcs}
In order to use both the previous support estimate and the previous nonzero coefficients' estimate, we can replace the initial LS estimate by a regularized LS estimate.
If training data is available to learn a linear prior model for signal coefficients' change, this can be done by replacing the LS estimator in step \ref{initls} of Sec. \ref{lscsalgo} by a Kalman filter (KF). The KF gives the optimal (in terms of minimizing the Bayesian MSE) regularization parameters when $|\Delta|=0$ and close-to-optimal ones if $|\Delta|$ is small. In this work, we consider the simplest linear model - an i.i.d. Gaussian random walk model. We develop KF CS-residual (KF-CS) for it in Sec. \ref{kfcsres}. Its stability is studied in Sec. \ref{kfcsstab}.%

%, i.e. $\xhat_{t,\text{init}}$ is now a Kalman filtered estimate and $\tty$ is now the Kalman filtering residual.
 %To be precise,   $(\xhat_{t,\text{init}})_T =  (I - K_{t,T} A_T) \xhat_{t-1} + K_{t,T} y_t$ and $(\xhat_{t,\text{init}})_{T^c} = 0$. The residual, $\tty = y_t - A_T (\xhat_{t,\text{init}})_T$. Here $K_{t,T}$ denotes the Kalman gain computed as explained in \cite{kfcsicip,kfcspap}.

\subsection{Gaussian random walk model with support additions}
\label{randwalk}
%We assume the following signal model.
\begin{sigmodel}
Assume the following model
\ben
\item  At $t=0$, $x_0$ is $S_0$ sparse with support $N_0$ and $(x_0)_{N_0} \sim \n(0,\sigma_{sys,0}^2 I)$. We assume that all elements of the support of $x_0$ get correctly estimated (by running CS with a large enough $n_0$) and there are no false detections. Thus at $t=1$, $T=\Nhat_0 = N_0$.
\item At every new addition time, $t_j = 1 + (j-1)d$, there are $S_a$ new additions to the support. Denote the set of indices of the currently added coefficients by $\add = \add(j)$.
\item There are no removals from the support, i.e. $N_{t-1} \subseteq N_t$.
\item Every new coefficient that gets added to the support starts from 0 and follows an independent Gaussian random walk model with zero drift and change variance $\sigma_{sys}^2$. Thus, we assume the following signal model:
\bea
%&& (x_0)_{N_0} \sim \n(0,\sigma_{sys}^2 I), \ \ (x_0)_{N_0^c} = 0   \nn \\
&& x_0 \sim \n(0,Q_0), \  Q_0 = \sigma_{sys,0}^2 I_{N_0}  \nn \\
&& x_t  =   x_{t-1} + \nu_t, \  \nu_t \sim \n(0,Q_t),   \  Q_t = \sigma_{sys}^2 I_{N_t},  \nn \\
&& N_{t-1} \subseteq N_t \ \text{and} \ |N_t \setminus N_{t-1}| = \left\{ \begin{array}{cc}
S_a \ & \ \text{if} \ t=t_j  \  \  \  \  \ \\
0 \ & \ \text{otherwise}  \  \  \  \  \
\end{array}
\right.
\label{sysmod}
\eea
where $I_T$ is defined in (\ref{defI}).

\item The maximum sparsity size of any $x_t$ is $\smax$. Thus there are a total of $K:=\lceil \frac{\smax-S_0}{S_a} \rceil$ addition times.%is in turn bounds the number of addition times to
\een
\label{randomwalk}
\end{sigmodel}
%Notice that $(x_t)_{N_t}$ is modeled as a random process, while we do not assume any model for support change (i.e. the $N_t$'s are deterministic but unknown). Such a model classifies as a  {\em partly-Bayesian} model.
%The above model cannot model removals from support, i.e. it needs $N_{t-1} \subseteq N_t$. This is because, in any realistic model for removing coefficients, only small coefficients will get removed, i.e. the set to be removed at time, $t$, will depend on the magnitude of the components of $(x_t)_{N_t}$ (which is modeled as a random vector). But, this will be inconsistent with our assumption of the $N_t$'s being non-random. % $N_{t} \setminus N_{t+1}$,

\subsection{Kalman Filtered CS-residual (KF-CS)}%using a Kalman filter (KF) along $T$, i.e. by
\label{kfcsres}
KF CS-residual (KF-CS) runs a KF for the system in (\ref{obsmod}), (\ref{sysmod}) but with $Q_t$ replaced by $\hat{Q}_t = \sigma_{sys}^2 I_{T}$ and computes the KF residual, $\tty$. The new additions, if any, to $T$, are detected by performing CS on $\tty$ and thresholding the output. If the support set changes, a final LS estimate can be computed using the new support estimate. If it does not change, we just use the KF output as the final estimate.
%$\xhat_{t|t-1}, \xhat_{t}$, predicted and updated state estimates at time $t$, the , $\Nhat_t$

Let $K_t$, $P_{t|t-1}$, $P_t$ denote the Kalman gain and the ``assumed" prediction and updated error covariance matrices used by the KF in KF-CS (we say ``assumed" since the KF does not always use the correct value of $Q_t$ and so $P_{t|t-1}$ or  $P_t$ are also not equal to the actual error covariances).

{\em We summarize KF-CS below.}

%{\em Initialization.} Set $\xhat_{0} = 0$, $\Nhat_0= \phi$, $P_0 = 0$. For $t > 0$ do,%
\noindent {\em Initialization ($t=0$): } At the initial time, $t=0$, we run simple CS with a large enough number of measurements, $n_0 > n$ (usually much larger), i.e. we solve (\ref{simplecs}) with $y=y_0$ and $A = A_0$ ($A_0$ will be an $n_0 \times m$ matrix). This is followed by support estimation and then LS estimation as in the Gauss-Dantzig selector. We denote the final output by $\xhat_0$ and its estimated support by $\Nhat_0$.
For $t>0$ do,
\ben
\item {\em Initial KF. } Let $T = \Nhat_{t-1}$. Run a Kalman prediction and update step using $\hat{Q}_t = \sigma_{sys}^2 I_{T}$ and compute the KF residual, $\tty$, i.e. compute
\label{initkf}
\bea
P_{t|t-1} \se P_{t-1} + \hat{Q}_t, \ \text{where} \ \hat{Q}_t :=\sigma_{sys}^2 I_{T}  \nn \\ % (P_{t-1} + \hat{Q}_t)
K_{t} \se P_{t|t-1} A' (AP_{t|t-1} A' + \sigma^2 I)^{-1}  \nn \\
%K_{t} \se ((P_{t-1} + \hat{Q}_t)^{-1} \sigma^2 + A'A)^{-1} A' \nn \\
P_t \se (I - K_{t} A) P_{t|t-1} \nn \\
\xhat_{t,\text{init}} \se (I - K_{t} A) \xhat_{t-1} + K_{t}  y_t \nn \\
\tty \se y_t - A \xhat_{t,\text{init}}    %y_t - A_{T} (\xhat_{t,\text{init}})_{T} %:= A \beta_t + w_t
\label{kftmp}
\eea

\item {\em CS-residual. } Do CS (Dantzig selector) on the KF residual, i.e.  solve (\ref{simplecs}) with $y= \tty$ and denote its output by $\betahat_t$. Compute $\xhat_{t,\CSres} = \xhat_{t,\text{init}} + \betahat_t$.% using (\ref{xhatcsres}).

\item {\em Additions and Final LS. } Estimate additions to $T$ to get $\Nhat_t$ as follows
\label{final_ls_step}
\bea
%\hat{\Delta} \se \{ i \in [1:m] : |(\xhat_{t,\CSres})_i| > \alpha \}, \nn \\
\Nhat_{t} \se T \cup \{ i \in [1:m] : |(\xhat_{t,\CSres})_i| > \alpha \}
\label{kfcs_detect}
\eea
If $\Nhat_t$ is equal to $\Nhat_{t-1}$,
\\ set $\xhat_{t}=\xhat_{t,\text{init}}$,
\\ else
\\ compute an LS estimate using $\Nhat_t$ and update $P_t$, i.e.
\bea
(\xhat_{t})_{\Nhat_t} \se {A_{\Nhat_t}}^\dag  y_t, \ \ (\xhat_{t})_{\Nhat_t^c} = 0 \nn \\ %{A_{\Nhat_t}}^\ddag '{A_{\Nhat_t}})^{-1}{A_{\Nhat_t}}'
(P_t)_{\Nhat_t,\Nhat_t} \se ({A_{\Nhat_t}}'{A_{\Nhat_t}})^{-1} \sigma^2
\label{finls_kf}
%\label{finalLS_kf}
\eea

\item Output $\xhat_t$ and $\hat{z}_t = \Phi \xhat_t$. Feedback $\xhat_t$, $P_t$, $\Nhat_t$.

%\item Output $\xhat_t$. Feedback $\xhat_t$, $P_t$, $\Nhat_t$. \item Set $t \leftarrow t+1$, go to step \ref{initkf}.%

\een
Increment $t$ and go to step \ref{initkf}.
\begin{remark}
For ease of notation, in (\ref{kftmp}), we write the KF equations for the entire $x_t$. But we actually run a reduced order KF for only $(x_t)_T$ at the current time (it is a dimension-varying KF), e.g. $(K_t)_{T^c,[1:n]} = 0$ and $(\xhat_t)_{T^c} = 0$.%, i.e. we actually have $(P_{t|t-1})_{[1:m],T^c} = (P_{t-1})_{[1:m],T^c} = 0$, $(P_{t|t-1})_{T^c,[1:m]} =(P_{t-1})_{T^c,[1:m]} = 0$, $(K_t)_{T^c,[1:n]} = 0$, $(\xhat_t)_{T^c} = 0$.For computational speedup, the reduced order KF should be explicitly implemented as explained in \cite{kfcsmri}.%The updates on $T^c$ are $(P_{t|t-1})_{[1:m],T^c} = (P_{t-1})_{[1:m],T^c} = 0$, $(P_{t|t-1})_{T^c,[1:m]} =(P_{t-1})_{T^c,[1:m]} = 0$, $(K_t)_{T^c,[1:m]} = 0$, $(\xhat_t)_{T^c} = (\xhat_{t-1})_{T^c} = 0$. %But, in implementation, for computational efficiency, one should perform all the matrix multiplications using the $n \times |T|$ nonzero sub-matrix of $A$ or the $|T| \times |T|$ nonzero sub-matrix of $P_{t|t-1}$ and so on (here $T \equiv T_{t-1}$ for (\ref{kftmp}) and $T \equiv T_{t}$ for (\ref{kfbig})).% For e.g., compute $(P_t)_{T,T} = [I - K_{t,T} A_T] (\Ppred)_{T,T}$ with $K_{t,T} = (({P_{t|t-1})_{T,T}}^{-1} \sigma_{obs}^2 + A_T'A_T)^{-1} A_T'$.% (needed especially when $m$ is very large)
\end{remark}

In practice, there typically will be true support removals. For such cases, a deletion step followed by another LS step can be added after step \ref{final_ls_step} (exactly as in LS-CS).%, exactly like step \ref{delete} of Sec. \ref{lscsalgo}.

The final LS step can be interpreted as reinitializing the KF with $P_{t|t-1} = \infty$ and $P_t$ given by (\ref{finls_kf}).%{A_{\Nhat_t}}^\dag$
%, $(K_t)_{\Nhat_t,[1:n]} =({A_{\Nhat_t}}'{A_{\Nhat_t}})^{-1}{A_{\Nhat_t}}'$, $(K_t)_{\Nhat_t^c,[1:n]}=0$

The KF in KF-CS does not always run with correct model parameters. Thus it is not clear if KF-CS always outperforms LS-CS. This is true at times when the support is accurately estimated and the KF has stabilized, e.g. see Fig.  \ref{kfcs_better_59}. A second situation is when $n$ is very small so that ${A_T}'A_T$ occasionally becomes badly conditioned. This leads to LS-CS instability, while KF-CS remains stable due to its use of previous signal estimates, e.g. see Fig. \ref{kfcs_better_40}.%


%then KF-CS for Signal Model \ref{randomwalk} gets to within a small error $\eps_{\text{err}}$ of the genie-KF estimate w.h.p..
\subsection{KF-CS Error Stability**}
\label{kfcsstab}
Consider the genie-aided KF, i.e. a KF which knows the true support $N_t$ at each $t$. It is the linear MMSE estimator of $x_t$ from $y_1, \dots y_t$ if the support sets, $N_t$, are known. %It would be the MMSE estimator if the observation noise were Gaussian.
%The genie-aided KF runs (\ref{kftmp}) with $\hat{Q}_t =  Q_t = \sigma_{sys}^2 I_{N_{t}}$ and uses $\xhat_{t,GAKF}=\xhat_{t,\text{init}}$ as its output.
In this section we find sufficient conditions under which, w.h.p., KF-CS for Signal Model \ref{randomwalk} gets to within a small error of the genie-KF, within a finite delay of the new addition time (the probability of this happening goes to one as the delay goes to infinity).
We show that this holds if the delay between addition times, $d$, is large enough; the addition threshold, $\alpha$, is large enough to ensure zero false additions; the noise is bounded and $n$ is large enough to ensure that $\smax \le \sinf$.
Since we assume a random walk model with zero drift, our computed bound on the high-probability detection delay is very loose.

%We prove the above result as follows.
We begin by giving Lemma \ref{finitedelay} which proves that, if the noise is bounded, $\smax \le \sinf$, and $\alpha$ is high enough, then the probability of false additions is zero. It also shows that if $d$ is large enough and if before the current addition time, $t_j$, the support is perfectly estimated, then w.p. $\ge 1-\eps$, all current additions will get detected by $t_j + \tau_{\dett}(\eps,S_a)$. $ \tau_{\dett}$ is what we call the high probability detection delay.

\begin{lemma}
Assume Signal Model \ref{randomwalk}. If
\ben
%\item $x_t$ follows the Signal Model \ref{randomwalk},
\item $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%\item we run KF-CS without the deletion step,
\item we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
\item the delay between addition times, $d > \tau_{\dett}(\eps,S_a)$, where
\bea
\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
\label{defteps}
\eea
where $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function,%
\een
then
\ben
\item there are no false additions, i.e. $\Nhat_t \subseteq N_t$
\item at each $t$, $\| x_t - \xhat_{t,\CSres}\|^2 \le B_*$
\item given that at $t = t_{j}-1$, $\Nhat_t=N_t$, then w.p. $\ge (1-\eps)$,  $\Nhat_t = N_t$  for all $t \in [t_j + \tau_{\dett}(\eps,S), t_{j+1}-1]$.% all additions are detected, i.e
\een
\label{finitedelay}
\end{lemma}
The proof is given in the Appendix.


Next we give Lemma \ref{kfinitwrong} which states that if the true support set does not change after a certain time, and if it gets correctly detected by a certain time, $t_*$, KF-CS will converge to the genie-KF in mean-square and hence also in probability.
\begin{lemma}
Assume that  $x_t$ follows Signal Model \ref{randomwalk}. Also assume that for all $t \ge t_*$, $\Nhat_t = N_t = N_*$ and assume that $\delta_{|N_*|} < 1$. The difference in the KF-CS and genie-KF estimates, $\diff_t :=\xhat_{t}-\xhat_{t,GAKF}$, converges to zero in mean square and hence also in probability. $\blacksquare$
\label{kfinitwrong}
\end{lemma}
The proof is similar to what should be a standard result for KF error convergence under wrong initial conditions, $\xhat_{t_*}, P_{t_*}$.
It should follow easily  from results in \cite{ekf}. But for ease of review, we give its complete proof in Appendix \ref{kfinitwrongproof}. %It is given in the Appendix \ref{kfinitwrongproof} (we could not find an appropriate citation and hence we give the proof).  of Lemma \ref{kfinitwrong}

A direct corollary of the above lemma is the following. %Its immediate corollary is that KF-CS will get to within a small error of the genie-KF if the delay between additions is large enough.
\begin{corollary}
Assume that $\Nhat_t = N_t = N_*$, for all $t \in [t_*, \ t_{**}]$. For a given $\eps, \eps_{\text{err}}$, there exists a $\tau_{KF}(\eps,\eps_{\text{err}},N_*)$ s.t. for all $t \in [t_* + \tau_{KF} , \ t_{**}]$, $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) > 1- \eps$. Clearly if $t_{**} < t_* + \tau_{KF}$, this is an empty interval.
\label{kfinitwrong_cor}
\end{corollary}

The KF-CS stability result follows directly by applying Lemma \ref{kfinitwrong} followed by Corollary \ref{kfinitwrong_cor} for each addition time.
\begin{theorem}[KF-CS Stability]
Assume that the assumptions of Lemma \ref{finitedelay} hold. Further assume that $d >\tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, where $\tau_{KF}$ is defined in Corollary \ref{kfinitwrong_cor}.
Then $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) \ge (1-\eps)^{j+1}$, for all $t \in [t_j + \tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j}), \ t_{j+1}-1]$.
\label{kfcs_stab}
\end{theorem}

Notice that $\tau_{KF}$ depends on the current support, $N_t=N_{t_j}$, for $t \in [t_j, t_{j+1}-1]$. Theorem \ref{kfcs_stab} says that if the time needed for the current KF to stabilize, $\tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, plus the high probability detection delay, $\tau_{\dett}(\eps,S_a)$, is smaller than $d$, then w.p. $\ge (1-\eps)^{j+1}$, KF-CS will stabilize to within a small error, $\eps_{\text{err}}$, of the genie-KF before the next addition time, $t_{j+1}$. If the current $\tau_{KF}$ is too large, this cannot be claimed.

A corollary of Theorem \ref{kfcs_stab} is that the same result holds for LS-CS (without the deletion step) stabilizing to the genie-LS. In fact, in this case $\tau_{KF}=0$ and $\eps_{\text{err}}=0$. This follows because LS-CS is equivalent to KF-CS with $\sigma_{sys}^2 = \infty$.
A second corollary is that after $t_K$, KF-CS will converge to the genie-KF in probability. The same is true for LS-CS without deletion. This is because after the last addition time, $t_K$, $N_t$ remains constant, i.e. $t_{K+1}=\infty$.% from Signal Model \ref{randomwalk},  of Theorem \ref{kfcs_stab}  converging to genie-LS

Notice that the above result is not as strong as the rest of the paper because it uses $\smax \le \sinf$ (instead of $S_a \le \sinf$).%while all the other results only need 

==> stability_kfcs_5.tex <==



\section{KF-CS: CS on KF Residual}% to improve the accuracy of simple CS
\label{supplem_kfcs}

Recall that LS-CS \cite{just_lscs} does not use the previous amplitude estimates, $(\xhat_{t-1})_T$, to improve the current estimate. In order to do this, we can replace the initial LS estimate by a regularized LS estimate.
%In order to use both the previous support estimate and the previous nonzero coefficients' estimate, we can replace the initial LS estimate by a regularized LS estimate.
If training data is available to learn a linear prior model for signal coefficients' change, this can be done by replacing the initial LS estimator  by a Kalman filtered (KF) estimate. The KF will give the optimal (in terms of minimizing the Bayesian MSE) regularization parameters if the size of the unknown support, $|\Delta|=0$ (and close-to-optimal ones if $|\Delta|$ is small). We assume a simple linear model - an i.i.d. Gaussian random walk model with non-decreasing support. This is specified in Sec. \ref{supplem_randwalk}. We develop KF CS-residual (KF-CS) for it in Sec. \ref{supplem_kfcsres}.%

%Its stability, under strong assumptions, is studied in Sec. \ref{supplem_kfcsstab}.%

%, i.e. $\xhat_{t,\text{init}}$ is now a Kalman filtered estimate and $\tty$ is now the Kalman filtering residual.
 %To be precise,   $(\xhat_{t,\text{init}})_T =  (I - K_{t,T} A_T) \xhat_{t-1} + K_{t,T} y_t$ and $(\xhat_{t,\text{init}})_{T^c} = 0$. The residual, $\tty = y_t - A_T (\xhat_{t,\text{init}})_T$. Here $K_{t,T}$ denotes the Kalman gain computed as explained in \cite{kfcsicip,kfcspap}.

\subsection{Gaussian random walk model with support additions}
\label{supplem_randwalk}
%We assume the following signal model.
\begin{sigmodel}
Assume the following model
\ben
\item  At $t=0$, $x_0$ is $S_0$ sparse with support $N_0$ and $(x_0)_{N_0} \sim \n(0,\sigma_{sys,0}^2 I)$.%We assume that all elements of the support of $x_0$ get correctly estimated (by running CS with a large enough $n_0$) and there are no false detections. Thus at $t=1$, $T=\Nhat_0 = N_0$.

\item At every new addition time, $t_j = 1 + jd$, for all $j=1,2,\dots K$ there are $S_a$ new additions to the support. Denote the set of indices of the currently added coefficients by $\add = \add(j)$.

\item There are no removals from the support, i.e. $N_{t-1} \subseteq N_t$.

\item The maximum sparsity size of  $x_t$ is $\smax$. Thus there are a total of $K:=\lceil \frac{\smax-S_0}{S_a} \rceil$ addition times.%is in turn bounds the number of addition times to

\item Every new coefficient that gets added to the support starts from 0 and follows an independent Gaussian random walk model with zero drift and change variance $\sigma_{sys}^2$, i.e. we assume the following ($I_T$ is defined in (\ref{defI})):
\bea
%&& (x_0)_{N_0} \sim \n(0,\sigma_{sys}^2 I), \ \ (x_0)_{N_0^c} = 0   \nn \\
&& x_0 \sim \n(0,Q_0), \  Q_0 = \sigma_{sys,0}^2 I_{N_0}  \nn \\
&& x_t  =   x_{t-1} + \nu_t, \  \nu_t \sim \n(0,Q_t),   \  Q_t = \sigma_{sys}^2 I_{N_t},  \nn \\
&& N_{t-1} \subseteq N_t \ \text{and} \ |N_t \setminus N_{t-1}| = \left\{ \begin{array}{cc}
S_a \ & \ \text{if} \ t=t_j  \  \  \  \  \ \\
0 \ & \ \text{otherwise}  \  \  \  \  \
\end{array}
\right.
\label{sysmod}
\eea
%where $I_T$ is defined in (\ref{defI}).

\een
\label{randomwalk}
\end{sigmodel}
In the above model, $(x_t)_{N_t}$ is modeled as a random process, while no model is assumed for for support change (i.e. the $N_t$'s are deterministic but unknown). Such a model classifies as a {\em partly-Bayesian} model.
The above model cannot model removals from support, i.e. it needs $N_{t-1} \subseteq N_t$. This is because, in any realistic model for removing coefficients, only small coefficients will get removed, i.e. the set to be removed at $t$ will be a function of the magnitude of the components of $(x_t)_{N_t}$ (which is modeled as a random vector). But, this will be inconsistent with our assumption of the $N_t$'s being non-random.% $N_{t} \setminus N_{t+1}$,

Notice that the above model contains just one unknown parameter (that is used by KF-CS), $\sigma_{sys}^2$, and hence it is easy to estimate its parameters from limited training data.

\subsection{KF-CS algorithm}%using a Kalman filter (KF) along $T$, i.e. by
\label{supplem_kfcsres}
KF CS-residual (KF-CS) runs a KF for the system in (\ref{obsmod}), (\ref{sysmod}) but with $Q_t$ replaced by $\hat{Q}_t = \sigma_{sys}^2 I_{T}$ and computes the KF residual, $\tty$. The new additions, if any, to $T$, are detected by performing CS on $\tty$ and thresholding the output. If the support set changes, a final LS estimate can be computed using the new support estimate. If it does not change, we just use the KF output as the final estimate and feed it back. %$\xhat_{t|t-1}, \xhat_{t}$, predicted and updated state estimates at time $t$, the , $\Nhat_t$

% If the support of $x_t$, $N_t$, were known at each $t$, and if the prior model given in the previous subsection holds, one could define a KF to get the linear MMSE estimate of $x_t$. When the support is unknown, one option is to do simple CS (Dantzig selector) at each time, i.e. solve (\ref{simplecs}) with $y=y_t$, followed by thresholding the output to estimate its support, and then do the same thing using the support estimate $\Nhat_t$ instead of $N_t$.
%But in doing so we are not using past observations to improve the CS estimate. Thus if $n$ is small, the CS estimate will be inaccurate, which in turn will mean that the support estimate (and thus the KF estimate) are all inaccurate.
%
%To use the information contained in past observations, along with the knowledge that support changes slowly, we propose the following idea. Assume for a moment that the support has not changed from $t-1$ to $t$. Use $T := \Nhat_{t-1}$ to compute an initial KF estimate and compute the KF residual. The KF estimate is computed as follows. Let $P_{t|t-1}$, $P_t$ and $K_t$ denote the ``assumed" prediction and updated error covariance matrices and the Kalman gain used by the KF in KF-CS (we say ``assumed" since the KF does not always use the correct value of $Q_t$ and so $P_{t|t-1}$ or $P_t$ are also not equal to the actual error covariances)  at time $t$.
%Compute the KF estimate $\xhat_{t,init}$ and the KF residual, $\tty$ as follows.
%\bea
%P_{t|t-1} \se P_{t-1} + \hat{Q}_t, \ \text{where} \ \hat{Q}_t :=\sigma_{sys}^2 I_{T}  \nn \\ % (P_{t-1} + \hat{Q}_t)
%K_{t} \se P_{t|t-1} A' (AP_{t|t-1} A' + \sigma^2 I)^{-1}  \nn \\
%%K_{t} \se ((P_{t-1} + \hat{Q}_t)^{-1} \sigma^2 + A'A)^{-1} A' \nn \\
%P_t \se (I - K_{t} A) P_{t|t-1} \nn \\
%\xhat_{t,\text{init}} \se (I - K_{t} A) \xhat_{t-1} + K_{t}  y_t \nn \\
%\tty \se y_t - A \xhat_{t,\text{init}}    %y_t - A_{T} (\xhat_{t,\text{init}})_{T} %:= A \beta_t + w_t
%\label{kftmp}
%\eea
%Notice that $\tty$ can be rewritten as $\tty = A \beta_t + w_t$ where
%\bea
%(\beta_t)_{(T \cup \Delta)^c} \se 0 \nn \\
%(\beta_t)_\Delta \se (x_t)_\Delta \nn \\
%(\beta_t)_T \se (x_t - \xhat_{t,\text{init}})_T \nn \\
%          \se [I - (K_t)_T A_T]A_\Delta x_\Delta + [I - A_T K_t] w \nn \\
%
%




In this work, the CS step in KF-CS is implemented using the Dantzig selector, i.e. it solves
\bea
\min_{\zeta} \|\zeta\|_1 \ \text{s.t.} \ \|A'(y - A \zeta)\|_\infty < \lambda %\lambda_m \sigma_{obs}, %\ \ \lambda := \sqrt{2 \log m}
\label{simplecs}
\eea
with $y$ replaced by the current KF residual, $\tty$.

Let $P_{t|t-1}$, $P_t$ and $K_t$ denote the ``assumed" prediction and updated error covariance matrices and the Kalman gain used by the KF in KF-CS (we say ``assumed" since the KF does not always use the correct value of $Q_t$ and so $P_{t|t-1}$ or $P_t$ are also not equal to the actual error covariances).

{\em We summarize the complete KF-CS below.}

%{\em Initialization.} Set $\xhat_{0} = 0$, $\Nhat_0= \phi$, $P_0 = 0$. For $t > 0$ do,% (usually much larger)
\noindent {\em Initialization ($t=0$): } At $t=0$, we run simple CS (Dantzig selector) with a large enough number of measurements, $n_0 > n$, i.e. we solve (\ref{simplecs}) with $y=y_0$ and $A = A_0$ ($A_0$ will be an $n_0 \times m$ matrix). This is followed by support estimation and then LS estimation as in the Gauss-Dantzig selector. We denote the final output by $\xhat_0$ and its estimated support by $\Nhat_0$.
For $t>0$ do,
\ben
\item {\em Initial KF. } Let $T = \Nhat_{t-1}$. Run a Kalman prediction and update step using $\hat{Q}_t = \sigma_{sys}^2 I_{T}$ and compute the KF residual, $\tty$, i.e. compute
\label{initkf}
\bea
P_{t|t-1} \se P_{t-1} + \hat{Q}_t, \ \text{where} \ \hat{Q}_t :=\sigma_{sys}^2 I_{T}  \nn \\ % (P_{t-1} + \hat{Q}_t)
K_{t} \se P_{t|t-1} A' (AP_{t|t-1} A' + \sigma^2 I)^{-1}  \nn \\
%K_{t} \se ((P_{t-1} + \hat{Q}_t)^{-1} \sigma^2 + A'A)^{-1} A' \nn \\
P_t \se (I - K_{t} A) P_{t|t-1} \nn \\
\xhat_{t,\text{init}} \se (I - K_{t} A) \xhat_{t-1} + K_{t}  y_t \nn \\
\tty \se y_t - A \xhat_{t,\text{init}}    %y_t - A_{T} (\xhat_{t,\text{init}})_{T} %:= A \beta_t + w_t
\label{kftmp}
\eea

\item {\em CS-residual. } Do CS (Dantzig selector) on the KF residual, i.e.  solve (\ref{simplecs})
%the following $$ \min_\beta \|\beta\|_1 \ \ s.t. \ \ \|A'(y-A\beta)\|_\infty \le \lambda $$
with $y= \tty$. Denote its output by $\betahat_t$. Compute $\xhat_{t,\CSres} = \xhat_{t,\text{init}} + \betahat_t$.% using (\ref{xhatcsres}).

\item {\em Additions and Final LS. } Estimate additions to $T$ to get $\Nhat_t$ as follows
\label{final_ls_step}
\bea
%\hat{\Delta} \se \{ i \in [1,m] : |(\xhat_{t,\CSres})_i| > \alpha \}, \nn \\
\Nhat_{t} \se T \cup \{ i \in [1,m] : |(\xhat_{t,\CSres})_i| > \alpha \} \nn
\label{kfcs_detect}
\eea
If $\Nhat_t$ is equal to $\Nhat_{t-1}$,
 set $\xhat_{t}=\xhat_{t,\text{init}}$,
\\ else,
\\ compute an LS estimate using $\Nhat_t$ and update $P_t$:
\bea
(\xhat_{t})_{\Nhat_t} \se {A_{\Nhat_t}}^\dag  y_t, \ \ (\xhat_{t})_{\Nhat_t^c} = 0 \nn \\ %{A_{\Nhat_t}}^\ddag '{A_{\Nhat_t}})^{-1}{A_{\Nhat_t}}'
(P_t)_{\Nhat_t,\Nhat_t} \se ({A_{\Nhat_t}}'{A_{\Nhat_t}})^{-1} \sigma^2
\label{finls_kf}
%\label{finalLS_kf}
\eea

\item Output $\xhat_t$ and $\hat{z}_t = \Phi \xhat_t$. Feedback $\xhat_t$, $P_t$, $\Nhat_t$.

%\item Output $\xhat_t$. Feedback $\xhat_t$, $P_t$, $\Nhat_t$. \item Set $t \leftarrow t+1$, go to step \ref{initkf}.%

\een
Increment $t$ and go to step \ref{initkf}.
\begin{remark}
For ease of notation, in (\ref{kftmp}), we write the KF equations for the entire $x_t$. But we actually run a reduced order KF for only $(x_t)_T$ at the current time. For example, notice that $(K_t)_{T^c,[1,n]} = 0$ or $(\xhat_t)_{T^c} = 0$.%, i.e. we actually have $(P_{t|t-1})_{[1,m],T^c} = (P_{t-1})_{[1,m],T^c} = 0$, $(P_{t|t-1})_{T^c,[1,m]} =(P_{t-1})_{T^c,[1,m]} = 0$, $(K_t)_{T^c,[1:n]} = 0$, $(\xhat_t)_{T^c} = 0$.For computational speedup, the reduced order KF should be explicitly implemented as explained in \cite{kfcsmri}.%The updates on $T^c$ are $(P_{t|t-1})_{[1,m],T^c} = (P_{t-1})_{[1,m],T^c} = 0$, $(P_{t|t-1})_{T^c,[1,m]} =(P_{t-1})_{T^c,[1,m]} = 0$, $(K_t)_{T^c,[1,m]} = 0$, $(\xhat_t)_{T^c} = (\xhat_{t-1})_{T^c} = 0$. %But, in implementation, for computational efficiency, one should perform all the matrix multiplications using the $n \times |T|$ nonzero sub-matrix of $A$ or the $|T| \times |T|$ nonzero sub-matrix of $P_{t|t-1}$ and so on (here $T \equiv T_{t-1}$ for (\ref{kftmp}) and $T \equiv T_{t}$ for (\ref{kfbig})).% For e.g., compute $(P_t)_{T,T} = [I - K_{t,T} A_T] (\Ppred)_{T,T}$ with $K_{t,T} = (({P_{t|t-1})_{T,T}}^{-1} \sigma_{obs}^2 + A_T'A_T)^{-1} A_T'$.% (needed especially when $m$ is very large)
\end{remark}% (it is a dimension-varying KF)

The final LS step can be interpreted as reinitializing the KF with $P_{t|t-1} = \infty$ and $P_t$ given by (\ref{finls_kf}). We use this in the basic algorithm above because it makes the analysis of stability easier (after a new addition time, we can first find sufficient conditions so that all elements of $\Delta$ get detected within a certain delay and then adapt stability results for the KF to show stability w.r.t. the genie-KF).

The KF in KF-CS does not always run with correct model parameters. Thus it is not clear if KF-CS always outperforms LS-CS. This will be true at times when the support is accurately estimated and the KF has stabilized. An important situation where this will hold is when $n$ is very small so that ${A_T}'A_T$ occasionally becomes badly conditioned. This will lead to LS-CS instability, while if this happens only occasionally, KF-CS will remains stable due to its use of previous signal estimates, e.g. see Fig. \ref{kfcs_better_40}.

Because of the above reason, when $n$ is small, it may also help to replace the final LS estimate by a final KF estimate.

%{A_{\Nhat_t}}^\dag$
%, $(K_t)_{\Nhat_t,[1:n]} =({A_{\Nhat_t}}'{A_{\Nhat_t}})^{-1}{A_{\Nhat_t}}'$, $(K_t)_{\Nhat_t^c,[1:n]}=0$
%, e.g. see Fig.  \ref{kfcs_better_59} in this figure KF is not optimal even when support correct



\subsection{Including a Deletion Step}
In practice, there will typically be true support removals. Also, unless the addition threshold is set very large, there will definitely be false detects by the KF-CS algorithm. In both cases, a deletion step needs to be added after step \ref{final_ls_step}. One also needs to update $P_t$ (zero out corresponding rows and columns). To be precise we can add the following after step \ref{final_ls_step}.
\bi
\item {\em Deletion Step. } Let $T = \Nhat_t$.
\ben
\item Compute the set to be deleted,
\bea
D:= \{i \in T: |(\xhat_t)_i| < \alpha_{del}\}
\eea
or threshold a time average of a set of past estimates to compute $D$.
\item Set $\Nhat_t : = T \setminus D$.
\item Set $(P_{t})_{D,[1,m]} = 0$ and $(P_{t})_{[1,m],D} = 0$. % $T_{tmp} = T_t$ and set $T_{t} = T_{tmp} \setminus \hat\Delta_C$.
\een
\ei
%, exactly like step \ref{delete} of Sec. \ref{lscsalgo}.  (as in LS-CS)


%then KF-CS for Signal Model \ref{randomwalk} gets to within a small error $\eps_{\text{err}}$ of the genie-KF estimate w.h.p..
\section{KF-CS Error Stability}
\label{supplem_kfcsstab}
Consider the genie-aided KF, i.e. a KF which knows the true support $N_t$ at each $t$. %and denote its estimate by $\xhat_{t,GAKF}$.
It is the linear MMSE estimator of $x_t$ from $y_1, \dots y_t$ if the support sets, $N_t$, are known. %It would be the MMSE estimator if the observation noise were Gaussian.
%The genie-aided KF runs (\ref{kftmp}) with $\hat{Q}_t =  Q_t = \sigma_{sys}^2 I_{N_{t}}$ and uses $\xhat_{t,GAKF}=\xhat_{t,\text{init}}$ as its output.
In this section, we find sufficient conditions under which, with high probability (w.h.p.), KF-CS for Signal Model \ref{randomwalk} gets to within a small error of the genie-KF, within a finite delay of the new addition time. The probability goes to one as the delay goes to infinity.
We show that this holds if the delay between addition times, $d$, is large enough; the addition threshold, $\alpha$, is large enough to ensure zero false detections; the noise is bounded and $n$ is large enough so that $\smax \le \sinf$.

{\em In this entire section, we only study the KF-CS algorithm given in Sec. \ref{supplem_kfcsres}.}

\subsection{The Stability Result}
We develop the result as follows. We begin by giving Lemma \ref{finitedelay} which shows two things. First, if the noise is bounded, $\smax \le \sinf$, and $\alpha$ is high enough, then the probability of false detections is zero. Second, if $d$ is large enough and if before the current addition time, $t_j$, the support was perfectly estimated, then w.p. $\ge 1-\eps$, all the current additions (which occurred at $t_j$) will get detected by $t_j + \tau_{\dett}(\eps,S_a)$. $ \tau_{\dett}$ is what we call the ``high probability detection delay".

\begin{lemma}
Assume Signal Model \ref{randomwalk}. If
\ben
%\item $x_t$ follows the Signal Model \ref{randomwalk},
\item $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%\item we run KF-CS without the deletion step,
\item we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
\item the delay between addition times, $d > \tau_{\dett}(\eps,S_a)$, where
\bea
\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
\label{defteps}
\eea
where $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function,%
\een
then
\ben
\item there are no false additions, i.e. $\Nhat_t \subseteq N_t$
\item at each $t$, $\| x_t - \xhat_{t,\CSres}\|^2 \le B_*$
\item given that at $t = t_{j}-1$, $\Nhat_t=N_t$, then w.p. $\ge (1-\eps)$,  $\Nhat_t = N_t$  for all $t \in [t_j + \tau_{\dett}(\eps,S), t_{j+1}-1]$.% all additions are detected, i.e
\een
\label{finitedelay}
\end{lemma}
The proof is given in Appendix \ref{finitedelay_proof}.

Next we give Lemma \ref{kfinitwrong} which states that if the true support set does not change after a certain time, and if it gets correctly detected by a certain time, $t_*$, KF-CS will converge to the genie-KF in mean-square and hence also in probability.
\begin{lemma}
Assume that  $x_t$ follows Signal Model \ref{randomwalk}. Also assume that for all $t \ge t_*$, $\Nhat_t = N_t = N_*$ and assume that $\delta_{|N_*|} < 1$. The difference in the KF-CS and genie-KF estimates, $\diff_t :=\xhat_{t}-\xhat_{t,GAKF}$, converges to zero in mean square and hence also in probability. $\blacksquare$
\label{kfinitwrong}
\end{lemma}
The proof is similar to what should be a standard result for KF error convergence under wrong initial conditions, $\xhat_{t_*}, P_{t_*}$.
It follows from the results of \cite{ekf}. The result may even exist in literature, although we were unable to find it in our search. For completeness and for ease of review, we give its complete proof in Appendix \ref{kfinitwrongproof}. %It is given in the Appendix \ref{kfinitwrongproof} (we could not find an appropriate citation and hence we give the proof).  of Lemma \ref{kfinitwrong}

A direct corollary of the above lemma is that KF-CS will get to within a small error of the genie-KF if the delay between additions is large enough. We state it below.
\begin{corollary}
Assume that $\Nhat_t = N_t = N_*$, for all $t \in [t_*, \ t_{**}]$. For a given $\eps, \eps_{\text{err}}$, there exists a $\tau_{KF}(\eps,\eps_{\text{err}},N_*)$ s.t. for all $t \in [t_* + \tau_{KF} , \ t_{**}]$, $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) > 1- \eps$. Clearly if $t_{**} < t_* + \tau_{KF}$, this is an empty interval.
\label{kfinitwrong_cor}
\end{corollary}

The KF-CS stability result follows directly by applying Lemma \ref{kfinitwrong} followed by Corollary \ref{kfinitwrong_cor} for each addition time, $t_j$.
\begin{theorem}[KF-CS Stability]
Let  $\diff_t:=\xhat_{t}-\xhat_{t,GAKF}$ where $\xhat_{t,GAKF}$ is the genie-KF estimate and $\xhat_t$ is the output of KF-CS. %($\xhat_{t,GAKF}$ is the genie-KF estimate). of Sec. \ref{kfcsres}
Under Signal Model \ref{randomwalk}, for a given $\eps, \eps_{\text{err}}$,%
\ben
\item {\em (initialization ($t=0$))} if all elements of $x_0$ get correctly detected and there are no false additions, i.e. $\Nhat_0 = N_0$,% at $t=1$, at $t=0$,
\item {\em (measurements)}  if $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%\item we run KF-CS without the deletion step,
\item {\em (algorithm)} if we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
\item {\em (signal model)} if the delay between addition times, $d > \tau_{\dett}(\eps,S_a)+ \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, where
\bea
\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
\label{defteps}
\eea
where $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function, and $\tau_{KF}$ is defined in Corollary \ref{kfinitwrong_cor} in the Appendix,
\een
then
\ben
\item  $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) \ge (1-\eps)^{j+1}$, for all $t \in [t_j + \tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j}), \ t_{j+1}-1]$.
\item w.p. $\ge (1-\eps)^K$, $|\Delta| \le S_a$ and $|\Delta_e|=0$ for all $t$.
\item  w.p. $\ge (1-\eps)^j$, $|\Delta|=0 = |\Delta_e|$ for all $t \in [t_j + \tau_{\dett}(\eps,S_a), t_{j+1}-1]$.
\een
\label{kfcs_stab}
\end{theorem}
The proof is given in Appendix \ref{append_kfcs}.

Notice that $\tau_{KF}$ depends on the current support, $N_t=N_{t_j}$, for $t \in [t_j, t_{j+1}-1]$. Theorem \ref{kfcs_stab} says that if the time needed for the current KF to stabilize, $\tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, plus the high probability detection delay,  $\tau_{\dett}(\eps,S_a)$, is smaller than $d$, then w.p. $\ge (1-\eps)^{j+1}$, KF-CS will stabilize to within a small error, $\eps_{\text{err}}$, of the genie-KF before the next addition time, $t_{j+1}$. If the current $\tau_{KF}$ is too large, this cannot be claimed.
Since the number of addition times is finite, $(1-\eps)^{j+1} \ge (1-\eps)^{K+1}$ (remains nonzero at all times).

A corollary of Theorem \ref{kfcs_stab} is that the same result holds for LS-CS (without the deletion step) stabilizing to the genie-LS. In fact, in this case $\tau_{KF}=0$ and $\eps_{\text{err}}=0$. %This follows because LS-CS is equivalent to KF-CS with $\sigma_{sys}^2 = \infty$.

A second corollary is that after $t_K$, KF-CS will converge to the genie-KF in probability.
This is because after $t_K$, $N_t$ remains constant, i.e. $t_{K+1}=\infty$. The same is true for LS-CS without deletion converging to to genie-LS.
% from Signal Model \ref{randomwalk},  of Theorem \ref{kfcs_stab}  converging to genie-LS the last addition time,

\subsection{Discussion}
Notice that our computed bound on the high-probability detection delay is very loose. This is because we assume a zero drift random walk model. Also, for the same reason, we need  $\smax \le \sinf$ (instead of $S_a \le \sinf$) which makes this result weaker than the stability result of \cite{just_lscs} which was proved for a deterministic signal model.

The reason for using the zero drift model is as follows. The drift is clearly not constant over time. To estimate a time-varying drift parameter, one would need to get multiple identically distributed training signal sequences, which is an impractical assumption in most cases.

Also note that while it is true that in practice, signals do not exactly follow the random walk model, but many real signal sequences can be modeled as follows. A new sparse basis coefficient (e.g. wavelet coefficient) will start from zero and slowly increase to a certain roughly constant value, i.e. it will follow a random walk model for sometime and then reach steady state in which it may remain constant or follow a stationary model. For such signal sequences, our result says that if, before reaching steady state, all coefficients become large enough to exceed the threshold plus upper bound on error, they will all get detected. And if this happens before the next addition time, KF-CS will remain stable.

Now to actually use the above signal model, random walk followed by stationary model (e.g. autoregressive model), one would either need to detect when a coefficient becomes stationary or one would need to know it ahead of time. The the former will typically be quite error prone while the latter is an impractical assumption. Hence, we just choose to just assume a random walk prior at all times while developing KF-CS.

An alternative approach that may yield a stronger theoretical result is to assume a random walk model with nonzero drift and one that becomes stationary after sometime, develop KF-CS for it, and study its stability.

%initially following a random walk model for sometime and then stabilizing to a stationary one. For example,

%We begin by giving Lemma \ref{finitedelay} which proves that, if the noise is bounded, $\smax \le \sinf$, and $\alpha$ is high enough, then the probability of false additions is zero. It also shows that if $d$ is large enough and if before the current addition time, $t_j$, the support is perfectly estimated, then w.p. $\ge 1-\eps$, all current additions will get detected by $t_j + \tau_{\dett}(\eps,S_a)$. $ \tau_{\dett}$ is what we call the high probability detection delay.
%
%\begin{lemma}
%Assume Signal Model \ref{randomwalk}. If
%\ben
%%\item $x_t$ follows the Signal Model \ref{randomwalk},
%\item $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%%\item we run KF-CS without the deletion step,
%\item we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
%\item the delay between addition times, $d > \tau_{\dett}(\eps,S_a)$, where
%\bea
%\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
%\label{defteps}
%\eea
%where $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function,%
%\een
%then
%\ben
%\item there are no false additions, i.e. $\Nhat_t \subseteq N_t$
%\item at each $t$, $\| x_t - \xhat_{t,\CSres}\|^2 \le B_*$
%\item given that at $t = t_{j}-1$, $\Nhat_t=N_t$, then w.p. $\ge (1-\eps)$,  $\Nhat_t = N_t$  for all $t \in [t_j + \tau_{\dett}(\eps,S), t_{j+1}-1]$.% all additions are detected, i.e
%\een
%\label{finitedelay}
%\end{lemma}
%The proof is given in the Appendix.
%
%
%Next we give Lemma \ref{kfinitwrong} which states that if the true support set does not change after a certain time, and if it gets correctly detected by a certain time, $t_*$, KF-CS will converge to the genie-KF in mean-square and hence also in probability.
%\begin{lemma}
%Assume that  $x_t$ follows Signal Model \ref{randomwalk}. Also assume that for all $t \ge t_*$, $\Nhat_t = N_t = N_*$ and assume that $\delta_{|N_*|} < 1$. The difference in the KF-CS and genie-KF estimates, $\diff_t :=\xhat_{t}-\xhat_{t,GAKF}$, converges to zero in mean square and hence also in probability. $\blacksquare$
%\label{kfinitwrong}
%\end{lemma}
%The proof is similar to what should be a standard result for KF error convergence under wrong initial conditions, $\xhat_{t_*}, P_{t_*}$.
%It should follow easily  from results in \cite{ekf}. But for ease of review, we give its complete proof in Appendix \ref{kfinitwrongproof}. %It is given in the Appendix \ref{kfinitwrongproof} (we could not find an appropriate citation and hence we give the proof).  of Lemma \ref{kfinitwrong}
%
%A direct corollary of the above lemma is the following. %Its immediate corollary is that KF-CS will get to within a small error of the genie-KF if the delay between additions is large enough.
%\begin{corollary}
%Assume that $\Nhat_t = N_t = N_*$, for all $t \in [t_*, \ t_{**}]$. For a given $\eps, \eps_{\text{err}}$, there exists a $\tau_{KF}(\eps,\eps_{\text{err}},N_*)$ s.t. for all $t \in [t_* + \tau_{KF} , \ t_{**}]$, $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) > 1- \eps$. Clearly if $t_{**} < t_* + \tau_{KF}$, this is an empty interval.
%\label{kfinitwrong_cor}
%\end{corollary}
%
%The KF-CS stability result follows directly by applying Lemma \ref{kfinitwrong} followed by Corollary \ref{kfinitwrong_cor} for each addition time.
%\begin{theorem}[KF-CS Stability]
%Assume that the assumptions of Lemma \ref{finitedelay} hold. Further assume that $d >\tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, where $\tau_{KF}$ is defined in Corollary \ref{kfinitwrong_cor}.
%Then $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) \ge (1-\eps)^{j+1}$, for all $t \in [t_j + \tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j}), \ t_{j+1}-1]$.
%\label{kfcs_stab}
%\end{theorem}
%
%Notice that $\tau_{KF}$ depends on the current support, $N_t=N_{t_j}$, for $t \in [t_j, t_{j+1}-1]$. Theorem \ref{kfcs_stab} says that if the time needed for the current KF to stabilize, $\tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, plus the high probability detection delay, $\tau_{\dett}(\eps,S_a)$, is smaller than $d$, then w.p. $\ge (1-\eps)^{j+1}$, KF-CS will stabilize to within a small error, $\eps_{\text{err}}$, of the genie-KF before the next addition time, $t_{j+1}$. If the current $\tau_{KF}$ is too large, this cannot be claimed.
%
%A corollary of Theorem \ref{kfcs_stab} is that the same result holds for LS-CS (without the deletion step) stabilizing to the genie-LS. In fact, in this case $\tau_{KF}=0$ and $\eps_{\text{err}}=0$. This follows because LS-CS is equivalent to KF-CS with $\sigma_{sys}^2 = \infty$.
%A second corollary is that after $t_K$, KF-CS will converge to the genie-KF in probability. The same is true for LS-CS without deletion. This is because after the last addition time, $t_K$, $N_t$ remains constant, i.e. $t_{K+1}=\infty$.% from Signal Model \ref{randomwalk},  of Theorem \ref{kfcs_stab}  converging to genie-LS
%
%Notice that the above result is not as strong as the rest of the paper because it uses $\smax \le \sinf$ (instead of $S_a \le \sinf$).%while all the other results only need 

==> stability_kfcs_6.tex <==



%Its stability, under strong assumptions, is studied in Sec. \ref{supplem_kfcsstab}.%

%, i.e. $\xhat_{t,\text{init}}$ is now a Kalman filtered estimate and $\tty$ is now the Kalman filtering residual.
 %To be precise,   $(\xhat_{t,\text{init}})_T =  (I - K_{t,T} A_T) \xhat_{t-1} + K_{t,T} y_t$ and $(\xhat_{t,\text{init}})_{T^c} = 0$. The residual, $\tty = y_t - A_T (\xhat_{t,\text{init}})_T$. Here $K_{t,T}$ denotes the Kalman gain computed as explained in \cite{kfcsicip,kfcspap}.


\section{Signal Model}
\label{priorsignalmodel}

%Recall that LS-CS \cite{just_lscs} does not use the previous amplitude estimates, $(\xhat_{t-1})_T$, to improve the current estimate. In order to do this, we can replace the initial LS estimate by a regularized LS estimate.
In order to use both the previous support estimate and the previous nonzero coefficients' estimate, we can replace the LS estimation step in LS-CS  by a regularized LS estimate. If training data is available to learn a linear prior model for signal coefficients' change, this can be done by replacing the initial LS estimator  by a Kalman filtered (KF) estimate. The KF will give the optimal (in terms of minimizing the Bayesian MSE) regularization parameters if the size of the unknown support, $|\Delta|=0$ (and close-to-optimal ones if $|\Delta|$ is small). We assume a simple linear model - an i.i.d. Gaussian random walk model with non-decreasing support. This is described below in Sec. \ref{supplem_randwalk}. Its pros and cons are discussed in Sec. \ref{whyrandwalk}.


\subsection{Gaussian Random Walk Model with Support Additions}
\label{supplem_randwalk}
We assume the following signal model.
\begin{sigmodel}
Assume the following model
\ben
\item  At $t=0$, $x_0$ is $S_0$ sparse with support $N_0$ and $(x_0)_{N_0} \sim \n(0,\sigma_{sys,0}^2 I)$.%We assume that all elements of the support of $x_0$ get correctly estimated (by running CS with a large enough $n_0$) and there are no false detections. Thus at $t=1$, $T=\Nhat_0 = N_0$.

\item At every new addition time, $t_j = 1 + jd$, for all $j=1,2,\dots K$ there are $S_a$ new additions to the support. Denote the set of indices of the currently added coefficients by $\add = \add(j)$.

\item There are no removals from the support, i.e. $N_{t-1} \subseteq N_t$.

\item The maximum sparsity size of  $x_t$ is $\smax$. Thus there are a total of $K:=\lceil \frac{\smax-S_0}{S_a} \rceil$ addition times.%is in turn bounds the number of addition times to

\item Every new coefficient that gets added to the support starts from 0 and follows an independent Gaussian random walk model with zero drift and change variance $\sigma_{sys}^2$, i.e. we assume the following: %($I_T$ is defined in (\ref{defI})):
\bea
%&& (x_0)_{N_0} \sim \n(0,\sigma_{sys}^2 I), \ \ (x_0)_{N_0^c} = 0   \nn \\
&& x_0 \sim \n(0,Q_0), \  Q_0 = \sigma_{sys,0}^2 I_{N_0}  \nn \\
&& x_t  =   x_{t-1} + \nu_t, \  \nu_t \sim \n(0,Q_t),   \  Q_t = \sigma_{sys}^2 I_{N_t},  \nn \\
&& |N_{t-1} \setminus N_t|=0 \ \text{and} \ |N_t \setminus N_{t-1}| = \left\{ \begin{array}{cc} %N_{t-1} \subseteq N_t
S_a \ & \ \text{if} \ t=t_j  \  \  \  \  \ \\
0 \ & \ \text{otherwise}  \  \  \  \  \
\end{array}
\right.
\label{sysmod}
\eea
%where $I_T$ is defined in (\ref{defI}).

\een
\label{randomwalk}
\end{sigmodel}

\subsection{Discussion}
\label{whyrandwalk}
In the above model, $(x_t)_{N_t}$ is modeled as a random process, while no model is assumed for support change (i.e. the $N_t$'s are deterministic but unknown). Such a model classifies as a {\em partly-Bayesian} model.
The above cannot model removals from support, i.e. it needs $N_{t-1} \subseteq N_t$. This is because, in any realistic model for removing coefficients, only small coefficients will get removed, i.e. the set to be removed at $t$ will be a function of the magnitude of the components of $(x_t)_{N_t}$ (which is modeled as a random vector). But this will be inconsistent with our assumption of $N_t$'s being non-random.% $N_{t} \setminus N_{t+1}$,

% Signal Model \ref{randomwalk}
A more accurate model than the above would be random walk with nonzero and time-varying drift. If perfect knowledge of the time-varying drift is available, the KF estimation error will reduce significantly. But, in practice, to estimate the time-varying drift values, one would need multiple identically distributed training signal sequences, which is an impractical assumption in most cases. On the other hand, in the above model the parameters are time-invariant and hence their values can be estimated from a single training sequence, e.g. see \cite{kfcsmri}.%In fact there is just a single parameter that is used by KF-CS - $\sigma_{sys}^2$. Hence its value can be accurately estimated from limited training data.%just a time-invariant parameter (that is used by the KF-CS algorithm), $\sigma_{sys}^2$. Hence it is easy to estimate the parameter value from limited training data.
%On the other hand, a random walk model with nonzero drift will make our estimation much more accurate if the parameters are correctly specified. But

%The reason for using the zero drift model is as follows. The drift is clearly not constant over time. To estimate a time-varying drift parameter, one would need to get multiple identically distributed training signal sequences, which is an impractical assumption in most cases.

Furthermore, a random walk model at all times is not a realistic signal model since it implies that signal power keeps increasing. The following is what is more realistic. A new sparse basis coefficient starts from zero and slowly increases to a certain roughly constant value, i.e. it follows a random walk model for sometime and then reaches steady state. Steady state can usually be modeled by a stationary model (e.g. i.i.d. or autoregressive model with nonzero mean given by the steady state value). %For such signal sequences, our result says that if, before reaching steady state, all coefficients become large enough to exceed the threshold plus upper bound on error, they will all get detected. And if this happens before the next addition time, KF-CS will remain stable.
Now to actually use the above signal model for defining KF-CS, one would either need to detect when a coefficient becomes stationary or one would need to know it ahead of time. The former will typically be very error prone while the latter is an impractical assumption. To avoid having to do this, we just assume a random walk model at all times.

In our simulations, we show that KF-CS designed for Signal Model \ref{randomwalk} works both for data generated from that model and for data generated from a more realistic bounded signal power signal model and one which includes both coefficient additions and removals. In \cite{kfcsmri}, we have demonstrated that such a KF-CS works even for actual medical image sequences.

 %(random walk followed by a stationary model)

%note that, while it is true that in practice, signals do not exactly follow the random walk model, but many



\section{Kalman filtered CS-residual (KF-CS)}% to improve the accuracy of simple CS
\label{supplem_kfcs}
We develop Kalman filtered CS-residual (KF-CS) for the signal model described above in Sec. \ref{supplem_kfcsres}. In Sec. \ref{whycsresworks}, we explain why doing CS on the KF residual is better than doing it on the observation (simple CS).


\subsection{KF-CS algorithm}%using a Kalman filter (KF) along $T$, i.e. by
\label{supplem_kfcsres}
KF CS-residual (KF-CS) runs a KF for the system in (\ref{obsmod}), (\ref{sysmod}) but with $Q_t$ replaced by $\hat{Q}_t = \sigma_{sys}^2 I_{T}$ and computes the KF residual, $\tty$. The new additions, if any, to $T$, are detected by performing CS on $\tty$ and thresholding the output. If the support set changes, a final LS estimate can be computed using the new support estimate. If it does not change, we just use the KF output as the final estimate and feed it back. %$\xhat_{t|t-1}, \xhat_{t}$, predicted and updated state estimates at time $t$, the , $\Nhat_t$

%If the support of $x_t$, $N_t$, were known at each $t$, and if the prior model given in the previous subsection holds, one could define a KF to get the linear MMSE estimate of $x_t$. When the support is unknown, one option is to do simple CS (Dantzig selector) at each time, i.e. solve (\ref{simplecs}) with $y=y_t$, followed by thresholding the output to estimate its support, and then do the same thing using the support estimate $\Nhat_t$ instead of $N_t$.
%But in doing so we are not using past observations to improve the CS estimate. Thus if $n$ is small, the CS estimate will be inaccurate, which in turn will mean that the support estimate (and thus the KF estimate) are all inaccurate.
%
%To use the information contained in past observations, along with the knowledge that support changes slowly, we propose the following idea. Assume for a moment that the support has not changed from $t-1$ to $t$. Use $T := \Nhat_{t-1}$ to compute an initial KF estimate and compute the KF residual. The KF estimate is computed as follows. Let $P_{t|t-1}$, $P_t$ and $K_t$ denote the ``assumed" prediction and updated error covariance matrices and the Kalman gain used by the KF in KF-CS (we say ``assumed" since the KF does not always use the correct value of $Q_t$ and so $P_{t|t-1}$ or $P_t$ are also not equal to the actual error covariances)  at time $t$.
%Compute the KF estimate $\xhat_{t,init}$ and the KF residual, $\tty$ as follows.
%\bea
%P_{t|t-1} \se P_{t-1} + \hat{Q}_t, \ \text{where} \ \hat{Q}_t :=\sigma_{sys}^2 I_{T}  \nn \\ % (P_{t-1} + \hat{Q}_t)
%K_{t} \se P_{t|t-1} A' (AP_{t|t-1} A' + \sigma^2 I)^{-1}  \nn \\
%%K_{t} \se ((P_{t-1} + \hat{Q}_t)^{-1} \sigma^2 + A'A)^{-1} A' \nn \\
%P_t \se (I - K_{t} A) P_{t|t-1} \nn \\
%\xhat_{t,\text{init}} \se (I - K_{t} A) \xhat_{t-1} + K_{t}  y_t \nn \\
%\tty \se y_t - A \xhat_{t,\text{init}}    %y_t - A_{T} (\xhat_{t,\text{init}})_{T} %:= A \beta_t + w_t
%\label{kftmp}
%\eea
%Notice that $\tty$ can be rewritten as $\tty = A \beta_t + w_t$ where
%\bea
%(\beta_t)_{(T \cup \Delta)^c} \se 0 \nn \\
%(\beta_t)_\Delta \se (x_t)_\Delta \nn \\
%(\beta_t)_T \se (x_t - \xhat_{t,\text{init}})_T \nn \\
%          \se [I - (K_t)_T A_T](x_{t} -  + [I - A_T K_t] w \nn \\


The CS step in KF-CS is implemented using the Dantzig selector \cite{dantzig}, i.e. it solves
\bea
\min_{\zeta} \|\zeta\|_1 \ \text{s.t.} \ \|A'(y - A \zeta)\|_\infty < \lambda %\lambda_m \sigma_{obs}, %\ \ \lambda := \sqrt{2 \log m}
\label{simplecs}
\eea
with $y$ replaced by the current KF residual.%, $\tty$, which is.

Let $P_{t|t-1}$, $P_t$ and $K_t$ denote the ``assumed" prediction and updated error covariance matrices and the Kalman gain used by the KF in KF-CS (we say ``assumed" since the KF does not always use the correct value of $Q_t$ and so $P_{t|t-1}$ or $P_t$ are also not equal to the actual error covariances).

{\em We summarize the complete KF-CS algorithm below.}

%{\em Initialization.} Set $\xhat_{0} = 0$, $\Nhat_0= \phi$, $P_0 = 0$. For $t > 0$ do,% (usually much larger)
\noindent {\em Initialization ($t=0$): } At $t=0$, we run simple CS (Dantzig selector) with a large enough number of measurements, $n_0 > n$, i.e. we solve (\ref{simplecs}) with $y=y_0$ and $A = A_0$ ($A_0$ will be an $n_0 \times m$ matrix). This is followed by support estimation and then LS estimation as in the Gauss-Dantzig selector. We denote the final output by $\xhat_0$ and its estimated support by $\Nhat_0$.
For $t>0$ do,
\ben
\item {\em Initial KF. } Let $T = \Nhat_{t-1}$. Run a Kalman prediction and update step using $\hat{Q}_t = \sigma_{sys}^2 I_{T}$ and compute the KF residual, $\tty$, i.e. compute
\label{initkf}
\bea
P_{t|t-1} \se P_{t-1} + \hat{Q}_t, \ \text{where} \ \hat{Q}_t :=\sigma_{sys}^2 I_{T}  \nn \\ % (P_{t-1} + \hat{Q}_t)
K_{t} \se P_{t|t-1} A' (AP_{t|t-1} A' + \sigma^2 I)^{-1}  \nn \\
%K_{t} \se ((P_{t-1} + \hat{Q}_t)^{-1} \sigma^2 + A'A)^{-1} A' \nn \\
P_t \se (I - K_{t} A) P_{t|t-1} \nn \\
\xhat_{t,\text{init}} \se (I - K_{t} A) \xhat_{t-1} + K_{t}  y_t \nn \\
\tty \se y_t - A \xhat_{t,\text{init}}    %y_t - A_{T} (\xhat_{t,\text{init}})_{T} %:= A \beta_t + w_t
\label{kftmp}
\eea

\item {\em CS-residual. } Do CS (Dantzig selector) on the KF residual, i.e.  solve (\ref{simplecs})
%the following $$ \min_\beta \|\beta\|_1 \ \ s.t. \ \ \|A'(y-A\beta)\|_\infty \le \lambda $$
with $y= \tty$. Denote its output by $\betahat_t$. Compute $\xhat_{t,\CSres} = \xhat_{t,\text{init}} + \betahat_t$.% using (\ref{xhatcsres}).

\item {\em Additions and Final LS. } Estimate additions to $T$ to get $\Nhat_t$ as follows
\label{final_ls_step}
\bea
%\hat{\Delta} \se \{ i \in [1,m] : |(\xhat_{t,\CSres})_i| > \alpha \}, \nn \\
\Nhat_{t} \se T \cup \{ i \in [1,m] : |(\xhat_{t,\CSres})_i| > \alpha \} \nn
\label{kfcs_detect}
\eea
If $\Nhat_t$ is equal to $\Nhat_{t-1}$,
 set $\xhat_{t}=\xhat_{t,\text{init}}$,
\\ else,
\\ compute an LS estimate using $\Nhat_t$ and update $P_t$, i.e.
\bea
(\xhat_{t})_{\Nhat_t} \se {A_{\Nhat_t}}^\dag  y_t, \ \ (\xhat_{t})_{\Nhat_t^c} = 0 \nn \\ %{A_{\Nhat_t}}^\ddag '{A_{\Nhat_t}})^{-1}{A_{\Nhat_t}}'
(P_t)_{\Nhat_t,\Nhat_t} \se ({A_{\Nhat_t}}'{A_{\Nhat_t}})^{-1} \sigma^2
\label{finls_kf}
%\label{finalLS_kf}
\eea

\item Output $\xhat_t$ and $\hat{z}_t = \Phi \xhat_t$. Feedback $\xhat_t$, $P_t$, $\Nhat_t$.

%\item Output $\xhat_t$. Feedback $\xhat_t$, $P_t$, $\Nhat_t$. \item Set $t \leftarrow t+1$, go to step \ref{initkf}.%

\een
Increment $t$ and go to step \ref{initkf}.


\begin{remark}[Reduced order KF]
For ease of notation, in (\ref{kftmp}), we write the KF equations for the entire $x_t$. But we actually run a reduced order KF for only $(x_t)_T$ at the current time, i.e. we actually have $(\xhat_t)_{T^c} = 0$, $(K_t)_{T^c,[1:n]} = 0$, $(P_{t|t-1})_{[1,m],T^c} = 0$, $ (P_{t-1})_{[1,m],T^c} = 0$, $(P_{t|t-1})_{T^c,[1,m]} = 0$, and $(P_{t-1})_{T^c,[1,m]} = 0$. For computational speedup, the reduced order KF should be explicitly implemented.% This is done in  \cite{kfcsmri}.%. For example, notice that $(K_t)_{T^c,[1,n]} = 0$ or $(\xhat_t)_{T^c} = 0$.
%
%as explained in \cite{kfcsmri}.%The updates on $T^c$ are $(P_{t|t-1})_{[1,m],T^c} = (P_{t-1})_{[1,m],T^c} = 0$, $(P_{t|t-1})_{T^c,[1,m]} =(P_{t-1})_{T^c,[1,m]} = 0$, $(K_t)_{T^c,[1,m]} = 0$, $(\xhat_t)_{T^c} = (\xhat_{t-1})_{T^c} = 0$. %But, in implementation, for computational efficiency, one should perform all the matrix multiplications using the $n \times |T|$ nonzero sub-matrix of $A$ or the $|T| \times |T|$ nonzero sub-matrix of $P_{t|t-1}$ and so on (here $T \equiv T_{t-1}$ for (\ref{kftmp}) and $T \equiv T_{t}$ for (\ref{kfbig})).% For e.g., compute $(P_t)_{T,T} = [I - K_{t,T} A_T] (\Ppred)_{T,T}$ with $K_{t,T} = (({P_{t|t-1})_{T,T}}^{-1} \sigma_{obs}^2 + A_T'A_T)^{-1} A_T'$.% (needed especially when $m$ is very large)
\end{remark}% (it is a dimension-varying KF)

\begin{remark}[KF-CS with deletion step]
In practice, there will typically be true support removals. Also, unless the addition threshold is set very large, there will also be false detects by the KF-CS algorithm. This necessitates a ``deletion" step to delete these elements from the support estimate. If this is not done ${A_{\Nhat_t}}$ may eventually become rank-deficient. This will make the observation model unobservable and in that case, the KF error may start diverging \cite{ekf}. %If this is not done, the estimated support size could keep increasing over time, eventually causing ${A_{\Nhat_t}}'{A_{\Nhat_t}}$ to become more and more ill-conditioned. This will  worsen the final LS estimate and also slowly worsen the initial KF estimate at future times.
%rank-deficient. This will make the observation model unobservable, and can result in the KF becoming unstable. Also of course the final LS estimate will %reduce the accuracy of both the initial KF estimate and the final LS estimate.
When a set of coefficients is deleted, one also needs to zero out corresponding rows and columns of $P_t$. Adding the following after step \ref{final_ls_step} is one simple way to do deletion.%needs to be added after step \ref{final_ls_step} of the KF-CS algorithm.
\bi
\item {\em Deletion Step. } Let $T = \Nhat_t$.
\ben
\item Compute the set to be deleted,
\bea
D:= \{i \in T: |(\xhat_t)_i| < \alpha_{del}\}
\eea
%or threshold a time average of a set of past estimates to compute $D$.
\item Set $\Nhat_t : = T \setminus D$.
\item Set $(P_{t})_{D,[1,m]} = 0$ and $(P_{t})_{[1,m],D} = 0$. % $T_{tmp} = T_t$ and set $T_{t} = T_{tmp} \setminus \hat\Delta_C$.
\\
\een
\ei
\end{remark}
%, exactly like step \ref{delete} of Sec. \ref{lscsalgo}.  (as in LS-CS)

\begin{remark}
The KF in KF-CS does not always run with correct model parameters. Thus it is not clear if KF-CS will always outperform LS-CS. This will be true at times when the support is accurately estimated and the KF has stabilized. Also, an important situation where this will hold is when $n$ is small so that ${A_T}'A_T$ will occasionally become ill-conditioned. This will lead to LS-CS instability, while if this happens {\em only occasionally}, KF-CS error will not increase. %will remains stable due to its use of previous signal estimates, e.g. see Fig. \ref{kfcs_better_40}.  since it does not invert ${A_T}'A_T$
Also because of the above reason, when $n$ is small, it can help to replace the final LS estimate in step \ref{final_ls_step} by a final KF estimate.
\end{remark}



%{A_{\Nhat_t}}^\dag$
%, $(K_t)_{\Nhat_t,[1:n]} =({A_{\Nhat_t}}'{A_{\Nhat_t}})^{-1}{A_{\Nhat_t}}'$, $(K_t)_{\Nhat_t^c,[1:n]}=0$
%, e.g. see Fig.  \ref{kfcs_better_59} in this figure KF is not optimal even when support correct

\subsection{CS-residual (CS on KF residual) versus simple CS}
\label{whycsresworks}
Notice that the KF residual, $\tty$, can be rewritten as $\tty = A \beta_t + w_t$ where
\bea
(\beta_t)_\Delta \se (x_t)_\Delta \nn \\
(\beta_t)_T \se (x_t - \xhat_{t,\text{init}})_T \nn \\
          \se [I - K_t A_T](x_{t} - \xhat_{t-1})_T - K_t A_T (x_t)_\Delta - K_t w_t \nn \\
(\beta_t)_{(T \cup \Delta)^c} \se 0
\label{defbeta}
\eea
where $T = \Nhat_{t-1}$ and $K_t \equiv  (K_t)_{T,[1,n]}$. As we explain in Appendix \ref{kfcsresbnd}, if (a) the support changes slowly enough, (b) the signal values change slowly enough, (c) the noise is small enough and (d) the previous reconstruction is accurate enough, $\beta_t$ will be small (compressible) along $T$. In other words, $\beta_t$ will be only $|\Delta|$-approximately-sparse. Thus doing CS on $\tty$ will incur much less error than doing CS on $y_t$ (simple CS) which needs to reconstruct a $|N_t|$-sparse signal, $x_t$.


%then KF-CS for Signal Model \ref{randomwalk} gets to within a small error $\eps_{\text{err}}$ of the genie-KF estimate w.h.p..
\section{KF-CS Error Stability}
\label{supplem_kfcsstab}
Consider the genie-aided KF, i.e. a KF which knows the true support $N_t$ at each $t$. %and denote its estimate by $\xhat_{t,GAKF}$.
It is the MMSE estimator of $x_t$ from $y_1, \dots y_t$ if the support sets, $N_t$, are known and the noise is Gaussian. %When the noise is arbitrary, it is still the best linear estimator.
%It would be the MMSE estimator if the observation noise were Gaussian.
%The genie-aided KF runs (\ref{kftmp}) with $\hat{Q}_t =  Q_t = \sigma_{sys}^2 I_{N_{t}}$ and uses $\xhat_{t,GAKF}=\xhat_{t,\text{init}}$ as its output.
In this section, we find sufficient conditions under which, with high probability (w.h.p.), KF-CS for Signal Model \ref{randomwalk} and observation model given by (\ref{obsmod}) gets to within a small error of the genie-KF for the same system, within a finite delay of the new addition time. %The probability goes to one as the delay goes to infinity.
We show that this holds if the delay between addition times, $d$, is large enough; the addition threshold, $\alpha$, is large enough to ensure zero false detects; the noise is bounded; and $n$ is large enough so that $\smax \le \sinf$.%

{\em We only study the basic KF-CS algorithm, i.e. the one without the deletion step and with using a final LS step.}
The final LS step can be interpreted as reinitializing the KF with $P_{t|t-1} = \infty$ and with $P_t$ and $\xhat_t$ given by (\ref{finls_kf}), whenever the support estimate, $\Nhat_t$, changes. This makes the analysis of stability easier. This becomes clear in the proof of Lemma \ref{kfinitwrong} given in Appendix \ref{kfinitwrongproof}.%(after a new addition time, we can first find sufficient conditions so that all elements of $\Delta$ get detected within a certain finite delay and then adapt stability results for KF for the sys).  given in Sec. \ref{supplem_kfcsres}
%Compared to using a final KF step,



\subsection{The Stability Result}
We develop the result as follows. We begin by giving Lemma \ref{finitedelay} which shows two things. First, if accurate initialization is assumed, if the noise is bounded and $\smax \le \sinf$, and if $\alpha$ is high enough, the probability of false detections is zero. Second, if the delay between addition times, $d > \tau_{\dett}(\eps,S_a)$, where $ \tau_{\dett}$ is what we call the ``high probability detection delay", the following holds. If before $t_j$, the support was perfectly estimated, then w.p. $\ge 1-\eps$, all the current additions (which occurred at $t_j$) will get detected by $t_j + \tau_{\dett}(\eps,S_a)$.% (the current addition time)

%$d$ is large enough and if before the current addition time, $t_j$, the support was perfectly estimated, then w.p. $\ge 1-\eps$, all the current additions (which occurred at $t_j$) will get detected by $t_j + \tau_{\dett}(\eps,S_a)$. $ \tau_{\dett}$ is what we call the ``high probability detection delay".

\begin{lemma}
Assume Signal Model \ref{randomwalk}. If
\ben
\item {\em (initialization ($t=0$))} all elements of $x_0$ get correctly detected and there are no false detects, i.e. $\Nhat_0 = N_0$,% at $t=1$, at $t=0$,
%\item $x_t$ follows the Signal Model \ref{randomwalk},
\item $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%\item we run KF-CS without the deletion step,
\item we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
\item the delay between addition times, $d > \tau_{\dett}(\eps,S_a)$, where
\bea
\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
\label{defteps}
\eea
where $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function,%
\een
then
\ben
\item there are no false detects, i.e. $\Nhat_t \subseteq N_t$
\item at each $t$, $\| x_t - \xhat_{t,\CSres}\|^2 \le B_*$
\item given that at $t = t_{j}-1$, $\Nhat_t=N_t$, then w.p. $\ge (1-\eps)$,  $\Nhat_t = N_t$  for all $t \in [t_j + \tau_{\dett}(\eps,S), t_{j+1}-1]$.% all additions are detected, i.e
\een
\label{finitedelay}
\end{lemma}
The proof is given in Appendix \ref{finitedelay_proof}. The initialization assumption is made only for simplicity. It can be easily satisfied by using $n_0 > n$ to be large enough.%

Next we give Lemma \ref{kfinitwrong} which states that if the true support set does not change after a certain time, $t_{nc}$, and if it gets correctly detected by a certain time, $t_* \ge t_{nc}$, then KF-CS will eventually converge to the genie-KF in mean-square and hence also in probability.
\begin{lemma}
Assume that  $x_t$ follows Signal Model \ref{randomwalk}. Also assume that for all $t \ge t_*$, $\Nhat_t = N_t = N_*$ and assume that $\delta_{|N_*|} < 1$. The difference in the KF-CS and genie-aided KF estimates, $\diff_t :=\xhat_{t}-\xhat_{t,GAKF}$, converges to zero in mean square and hence also in probability. $\blacksquare$
\label{kfinitwrong}
\end{lemma}
The proof is similar to what should be a standard result for the error between a KF run with wrong initial conditions (here, KF-CS for $t \ge t_*$  with $\xhat_{t_*}, P_{t_*}$ being the initial conditions) and a KF run with correct initial conditions (here, the genie KF) to converge to zero with time. %KF error convergence under wrong initial conditions, $\xhat_{t_*}, P_{t_*}$. It follows from the results of \cite{ekf}.
We could not find the exact result proved anywhere (we only found results for $P_{t|t-1}$, and hence for $P_t$ and $K_t$, to converge to a steady state value computed using the Riccatti equation) and hence for completeness we just give our proof in Appendix \ref{kfinitwrongproof}.%It is given in the Appendix \ref{kfinitwrongproof} (we could not find an appropriate citation and hence we give the proof).  of Lemma \ref{kfinitwrong}

A direct corollary of the above lemma is that, w.h.p., KF-CS will get to within a small error of the genie-KF if the delay between addition times is large enough. We state it here.
\begin{corollary}
Assume that $\Nhat_t = N_t = N_*$, for all $t \in [t_*, \ t_{**}]$. For a given $\eps, \eps_{\text{err}}$, there exists a $\tau_{KF}(\eps,\eps_{\text{err}},N_*)$ s.t. for all $t \in [t_* + \tau_{KF} , \ t_{**}]$, $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) > 1- \eps$. Clearly if $t_{**} < t_* + \tau_{KF}$, this is an empty interval.
\label{kfinitwrong_cor}
\end{corollary}

Our stability result then follows by applying Lemma \ref{kfinitwrong} followed by Corollary \ref{kfinitwrong_cor} for each addition time, $t_j$.%
\begin{theorem}[KF-CS Stability]
Let  $\diff_t:=\xhat_{t}-\xhat_{t,GAKF}$ where $\xhat_{t,GAKF}$ is the genie-aided KF estimate and $\xhat_t$ is the output of KF-CS. %($\xhat_{t,GAKF}$ is the genie-KF estimate). of Sec. \ref{kfcsres}
Under Signal Model \ref{randomwalk}, for a given $\eps, \eps_{\text{err}}$,%
\ben
\item {\em (initialization ($t=0$))} if all elements of $x_0$ get correctly detected and there are no false detects, i.e. $\Nhat_0 = N_0$,% at $t=1$, at $t=0$,
\item {\em (measurements)}  if $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%\item we run KF-CS without the deletion step,
\item {\em (algorithm)} if we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
\item {\em (signal model)} if the delay between addition times, $d > \tau_{\dett}(\eps,S_a)+ \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, where
%\bea
%\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
%\label{defteps}
%\eea
%where  $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function,
$\tau_{\dett}(.,.)$ is defined in (\ref{defteps}) in Lemma \ref{finitedelay} and and $\tau_{KF}(.,.,.)$ in Corollary \ref{kfinitwrong_cor},%
\een
then
\ben
\item  $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) > (1-\eps)^{j+1}$, for all $t \in [t_j + \tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j}), \ t_{j+1}-1]$.
\item w.p. $\ge (1-\eps)^K$, $|\Delta| \le S_a$ and $|\Delta_e|=0$ for all $t$, and
\item  w.p. $\ge (1-\eps)^K$, %(1-\eps)^j \ge
$|\Delta|=0 = |\Delta_e|$ for all $t \in [t_j + \tau_{\dett}(\eps,S_a), t_{j+1}-1]$. %for all $j=1,\dots K$.

\een
\label{kfcs_stab}
\end{theorem}
The proof is given in Appendix \ref{append_kfcs}.


%A corollary of Theorem \ref{kfcs_stab} is that the same result holds for LS-CS (without the deletion step) stabilizing to the genie-LS. In fact, in this case $\tau_{KF}=0$ and $\eps_{\text{err}}=0$. %This follows because LS-CS is equivalent to KF-CS with $\sigma_{sys}^2 = \infty$.

A direct corollary of Theorem \ref{kfcs_stab} is that after $t_K$, KF-CS will converge to the genie-KF in probability.
This is because after $t_K$, $N_t$ remains constant, i.e. $t_{K+1}=\infty$. %The same is true for LS-CS without deletion converging to to genie-LS.
% from Signal Model \ref{randomwalk},  of Theorem \ref{kfcs_stab}  converging to genie-LS the last addition time,


\subsection{Discussion}
Notice that $\tau_{KF}$ depends on the current support, $N_t=N_{t_j}$, for $t \in [t_j, t_{j+1}-1]$. Theorem \ref{kfcs_stab} says that if the time needed for the current KF to stabilize, $\tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, plus the high probability detection delay,  $\tau_{\dett}(\eps,S_a)$, is smaller than $d$, then w.p. $\ge (1-\eps)^{j+1}$, KF-CS will stabilize to within a small error, $\eps_{\text{err}}$, of the genie-KF before the next addition time, $t_{j+1}$. If the current $\tau_{KF}$ is too large, this cannot be claimed.
Furthermore, w.h.p., the unknown support size, $|\Delta|$ remains bounded by $S_a$.
%Since the number of addition times is finite, $(1-\eps)^{j+1} \ge (1-\eps)^{K+1}$ (remains nonzero at all times).

As explained in Sec. \ref{whyrandwalk}, most signals do not follow a random walk model forever - a new coefficient may start with following a random walk model until it reaches steady state. In this case, our result can be modified to claim that if, before reaching steady state, all coefficients become large enough to exceed the threshold plus upper bound on error, and if this happens before the next addition time, KF-CS remains stable.%they will all get detected. (starts following a stationary model)

Our result is weaker compared to the stability result for LS-CS in \cite{just_lscs} - it needs $\smax \le \sinf$ (while the LS-CS result only needs $S_a \le \sinf$) and the computed high-probability detection delay is also quite loose\footnote{In fact our result may even go through if the CS-residual step was replaced by simple CS.}. This is due to two main reasons. One is that we use a random walk model with zero drift as the signal model both for defining KF-CS and for analyzing it, while LS-CS does not use a signal model for the algorithm and uses a model with nonzero drift for the analysis. The reason for choosing the zero drift random walk model is explained in Sec. \ref{whyrandwalk}. %The reason we use this model is because the KF definition uses the signal model and a random walk model with nonzero drift is impractical to estimate parameters of (as explained in Sec. \ref{model}).
The second and more important reason is that bounding KF error is more difficult than bounding LS error. This is because the KF error, and hence also the (KF)CS-residual step error, depends on the previous reconstruction error and this makes the approach of \cite{just_lscs} difficult to adapt. On the other hand (LS)CS-residual error only depends on the size of $T$ and $\Delta$ and as long as we can get a  bound on their sizes that is independent of time, we can also do the same for (LS)CS-residual error.%


%While it is true that in practice, signals do not exactly follow the random walk model, but many real signal sequences can be modeled as follows. A new sparse basis coefficient will start from zero and slowly increase to a certain roughly constant value, i.e. it will follow a random walk model for sometime and then reach steady state. In steady state, it may follow a stationary model (e.g. i.i.d. or autoregressive model with nonzero mean given by the steady state value). %For such signal sequences, our result says that if, before reaching steady state, all coefficients become large enough to exceed the threshold plus upper bound on error, they will all get detected. And if this happens before the next addition time, KF-CS will remain stable.
%Now to actually use the above signal model (random walk followed by a stationary model)  both for defining KF-CS and for analyzing it, one would either need to detect when a coefficient becomes stationary or one would need to know it ahead of time. The former will typically be very error prone while the latter is an impractical assumption. Hence, we just choose to just assume a random walk prior at all times while developing KF-CS.



%\subsection{Discussion}
%Notice that our computed bound on the high-probability detection delay is very loose. This is because we assume a zero drift random walk model. Also, for the same reason, we need  $\smax \le \sinf$ (instead of $S_a \le \sinf$) which makes this result weaker than the stability result of \cite{just_lscs} which was proved for a deterministic signal model.
%
%The reason for using the zero drift model is as follows. The drift is clearly not constant over time. To estimate a time-varying drift parameter, one would need to get multiple identically distributed training signal sequences, which is an impractical assumption in most cases.
%
%Also note that while it is true that in practice, signals do not exactly follow the random walk model, but many real signal sequences can be modeled as follows. A new sparse basis coefficient (e.g. wavelet coefficient) will start from zero and slowly increase to a certain roughly constant value, i.e. it will follow a random walk model for sometime and then reach steady state in which it may remain constant or follow a stationary model. For such signal sequences, our result says that if, before reaching steady state, all coefficients become large enough to exceed the threshold plus upper bound on error, they will all get detected. And if this happens before the next addition time, KF-CS will remain stable.
%
%Now to actually use the above signal model, random walk followed by stationary model (e.g. autoregressive model), one would either need to detect when a coefficient becomes stationary or one would need to know it ahead of time. The the former will typically be quite error prone while the latter is an impractical assumption. Hence, we just choose to just assume a random walk prior at all times while developing KF-CS.
%
%An alternative approach that may yield a stronger theoretical result is to assume a random walk model with nonzero drift and one that becomes stationary after sometime, develop KF-CS for it, and study its stability.

%initially following a random walk model for sometime and then stabilizing to a stationary one. For example,

%We begin by giving Lemma \ref{finitedelay} which proves that, if the noise is bounded, $\smax \le \sinf$, and $\alpha$ is high enough, then the probability of false additions is zero. It also shows that if $d$ is large enough and if before the current addition time, $t_j$, the support is perfectly estimated, then w.p. $\ge 1-\eps$, all current additions will get detected by $t_j + \tau_{\dett}(\eps,S_a)$. $ \tau_{\dett}$ is what we call the high probability detection delay.
%
%\begin{lemma}
%Assume Signal Model \ref{randomwalk}. If
%\ben
%%\item $x_t$ follows the Signal Model \ref{randomwalk},
%\item $\smax \le \sinf$ and $\|w\|_\infty \le \lambda/\|A\|_1$,
%%\item we run KF-CS without the deletion step,
%\item we set $\alpha^2  = B_* := C_1(\smax) \smax \lambda^2$, where $C_1(S)$ is defined in Theorem 1.1. of \cite{dantzig},
%\item the delay between addition times, $d > \tau_{\dett}(\eps,S_a)$, where
%\bea
%\tau_{\dett}(\eps,S):=\lceil  \frac{4 B_*}{ \sigma_{sys}^2 [\Q^{-1}(\frac{ (1- \eps)^{1/S} }{2})]^2 } \rceil - 1
%\label{defteps}
%\eea
%where $\lceil \cdot \rceil$ denotes the greatest integer function and $\Q(z):= \int_{z}^\infty (1/\sqrt{2\pi}) e^{-x^2/2} dx$ is Gaussian Q-function,%
%\een
%then
%\ben
%\item there are no false additions, i.e. $\Nhat_t \subseteq N_t$
%\item at each $t$, $\| x_t - \xhat_{t,\CSres}\|^2 \le B_*$
%\item given that at $t = t_{j}-1$, $\Nhat_t=N_t$, then w.p. $\ge (1-\eps)$,  $\Nhat_t = N_t$  for all $t \in [t_j + \tau_{\dett}(\eps,S), t_{j+1}-1]$.% all additions are detected, i.e
%\een
%\label{finitedelay}
%\end{lemma}
%The proof is given in the Appendix.
%
%
%Next we give Lemma \ref{kfinitwrong} which states that if the true support set does not change after a certain time, and if it gets correctly detected by a certain time, $t_*$, KF-CS will converge to the genie-KF in mean-square and hence also in probability.
%\begin{lemma}
%Assume that  $x_t$ follows Signal Model \ref{randomwalk}. Also assume that for all $t \ge t_*$, $\Nhat_t = N_t = N_*$ and assume that $\delta_{|N_*|} < 1$. The difference in the KF-CS and genie-KF estimates, $\diff_t :=\xhat_{t}-\xhat_{t,GAKF}$, converges to zero in mean square and hence also in probability. $\blacksquare$
%\label{kfinitwrong}
%\end{lemma}
%The proof is similar to what should be a standard result for KF error convergence under wrong initial conditions, $\xhat_{t_*}, P_{t_*}$.
%It should follow easily  from results in \cite{ekf}. But for ease of review, we give its complete proof in Appendix \ref{kfinitwrongproof}. %It is given in the Appendix \ref{kfinitwrongproof} (we could not find an appropriate citation and hence we give the proof).  of Lemma \ref{kfinitwrong}
%
%A direct corollary of the above lemma is the following. %Its immediate corollary is that KF-CS will get to within a small error of the genie-KF if the delay between additions is large enough.
%\begin{corollary}
%Assume that $\Nhat_t = N_t = N_*$, for all $t \in [t_*, \ t_{**}]$. For a given $\eps, \eps_{\text{err}}$, there exists a $\tau_{KF}(\eps,\eps_{\text{err}},N_*)$ s.t. for all $t \in [t_* + \tau_{KF} , \ t_{**}]$, $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) > 1- \eps$. Clearly if $t_{**} < t_* + \tau_{KF}$, this is an empty interval.
%\label{kfinitwrong_cor}
%\end{corollary}
%
%The KF-CS stability result follows directly by applying Lemma \ref{kfinitwrong} followed by Corollary \ref{kfinitwrong_cor} for each addition time.
%\begin{theorem}[KF-CS Stability]
%Assume that the assumptions of Lemma \ref{finitedelay} hold. Further assume that $d >\tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, where $\tau_{KF}$ is defined in Corollary \ref{kfinitwrong_cor}.
%Then $Pr(\|\diff_t\|^2 \le \eps_{\text{err}}) \ge (1-\eps)^{j+1}$, for all $t \in [t_j + \tau_{\dett}(\eps,S_a) + \tau_{KF}(\eps,\eps_{\text{err}},N_{t_j}), \ t_{j+1}-1]$.
%\label{kfcs_stab}
%\end{theorem}
%
%Notice that $\tau_{KF}$ depends on the current support, $N_t=N_{t_j}$, for $t \in [t_j, t_{j+1}-1]$. Theorem \ref{kfcs_stab} says that if the time needed for the current KF to stabilize, $\tau_{KF}(\eps,\eps_{\text{err}},N_{t_j})$, plus the high probability detection delay, $\tau_{\dett}(\eps,S_a)$, is smaller than $d$, then w.p. $\ge (1-\eps)^{j+1}$, KF-CS will stabilize to within a small error, $\eps_{\text{err}}$, of the genie-KF before the next addition time, $t_{j+1}$. If the current $\tau_{KF}$ is too large, this cannot be claimed.
%
%A corollary of Theorem \ref{kfcs_stab} is that the same result holds for LS-CS (without the deletion step) stabilizing to the genie-LS. In fact, in this case $\tau_{KF}=0$ and $\eps_{\text{err}}=0$. This follows because LS-CS is equivalent to KF-CS with $\sigma_{sys}^2 = \infty$.
%A second corollary is that after $t_K$, KF-CS will converge to the genie-KF in probability. The same is true for LS-CS without deletion. This is because after the last addition time, $t_K$, $N_t$ remains constant, i.e. $t_{K+1}=\infty$.% from Signal Model \ref{randomwalk},  of Theorem \ref{kfcs_stab}  converging to genie-LS
%
%Notice that the above result is not as strong as the rest of the paper because it uses $\smax \le \sinf$ (instead of $S_a \le \sinf$).%while all the other results only need 

==> table.tex <==
\begin{table*}[ht!]
\caption{Comparing normalized MSE of CS-residual (with $\lambda=4\sigma$) with that of CS (Dantzig Selector (DS)) with three different $\lambda$'s. We used $m=200$, $|N|=20$, $|\Delta|=|\Delta_e|=2$. Comparison shown for three choices of $n=45,59,100$ in the three tables below.}% and different $\sigma$'s for each $n$
\centerline{
\begin{tabular}{|l|l|l|l|l|}
\hline
\hline
($n=45$) & $n$=45 & $n$=45 & $n$=45  & $n$=45 \\
             & $\sigma$=0.04 &  $\sigma$=0.09 &  $\sigma$=0.18 & $\sigma$=0.44 \\
 \hline
DS,$\lambda$=$12\sigma$ & 0.8235   &   0.8952  &    0.9794    &  1.0000 \\
 \hline
DS,$\lambda$=$4\sigma$ & 0.7994   &   0.8320    &  0.8642   &   0.9603 \\
\hline
DS,$\lambda$=$0.4\sigma$  & 0.8071   &   0.8476   &   0.8762  &    1.0917 \\
\hline
%Gauss-DS \\ \hline
CS-residual             &      0.1397   &   0.1685   &   0.2270    &  0.5443 \\
%\hline LS-CS  & 0.0091  &    0.0949   &   0.2247    &  0.5443 \\
\hline
\hline
\end{tabular}
\hspace{0.05in}
\begin{tabular}{|l|l|l|l|l|}
\hline \hline
($n=59$) & $n$=59 & $n$=59 & $n$=59  & $n$=59 \\
                & $\sigma$=0.04 &  $\sigma$=0.09 &  $\sigma$=0.18 & $\sigma$=0.44 \\
 \hline
DS,$\lambda$=$12\sigma$ & 0.7572   &   0.8402   &   0.9937   &   1.0000 \\
 \hline
DS,$\lambda$=$4\sigma$ & 0.6545  &    0.6759  &    0.7991    &  0.9607  \\
\hline
DS,$\lambda$=$0.4\sigma$ & 0.5375   &   0.5479   &   0.7086    &  1.0525 \\
\hline
CS-residual & 0.0866       &  0.1069  &    0.1800   &   0.4102 \\ %,$\lambda$=$4\sigma$
%\hline LS-CS & 0.0044      &   0.0205   &   0.1793    &  0.4102 \\
\hline
\hline
\end{tabular}
\hspace{0.05in}
\begin{tabular}{|l|l|l|}
\hline \hline%($n=100$)
($n=100$) & $n$=100 & $n$=100 \\ % & $n$=100  & $n$=100
    & $\sigma$=0.04 &  $\sigma$=0.09 \\ % &  $\sigma$ = 0.18 & $\sigma$=0.44 \\
 \hline
DS,$\lambda$=$12\sigma$ &  0.5856   &   0.8547  \\  % 0.9977    1.0000 \\
\hline
DS,$\lambda$=$4\sigma$ & 0.2622   &  0.4975   \\ % 0.6956    0.9677 \\
\hline
DS,$\lambda$=$0.4\sigma$ & 0.0209  &   0.0929   \\ % 0.3316    1.0687 \\
\hline
CS-residual             & 0.0402   &  0.0687 \\  % 0.1389    0.3653 \\%,$\lambda$=$4\sigma$
%\hline LS-CS               & 0.0032   &  0.0128   \\ %0.1156    0.3653  \\
\hline
\hline
\end{tabular}
}
\label{static_table}
\end{table*}

